Measurement of prompt $D^+$ and $D^+_{s}$ production in $p\mathrm{Pb}$ collisions at $\sqrt {s_{\mathrm{NN}}}=5.02\,$TeV

The production of prompt $D^+$ and $D^+_{s}$ mesons is studied in proton-lead collisions at a centre-of-mass energy of $\sqrt {s_{\mathrm{NN}}}=5.02\,$TeV. The data sample corresponding to an integrated luminosity of $(1.58\pm0.02)\mathrm{nb}^{-1}$ is collected by the LHCb experiment at the LHC. The differential production cross-sections are measured using $D^+$ and $D^+_{s}$ candidates with transverse momentum in the range of $0<p_{\mathrm{T}} <14\,\mathrm{GeV}/c$ and rapidities in the ranges of $1.5<y^*<4.0$ and $-5.0<y^*<-2.5$ in the nucleon-nucleon centre-of-mass system. For both particles, the nuclear modification factor and the forward-backward production ratio are determined. These results are compared with theoretical models that include initial-state nuclear effects. In addition, measurements of the cross-section ratios between $D^+$, $D^+_{s}$ and $D^0$ mesons are presented, providing a baseline for studying the charm hadronization in lead-lead collisions at LHC energies.

==> Authorship_LHCb-PAPER-2023-006-arXiv.tex <==
LHCb collaboration:
R. Aaij,
A.S.W. Abdelmotteleb,
C. Abellan Beteta,
F. Abudin{\'e}n,
T. Ackernley,
B. Adeva,
M. Adinolfi,
P. Adlarson,
H. Afsharnia,
C. Agapopoulou,
C.A. Aidala,
Z. Ajaltouni,
S. Akar,
K. Akiba,
P. Albicocco,
J. Albrecht,
F. Alessio,
M. Alexander,
A. Alfonso Albero,
Z. Aliouche,
P. Alvarez Cartelle,
R. Amalric,
S. Amato,
J.L. Amey,
Y. Amhis,
L. An,
L. Anderlini,
M. Andersson,
A. Andreianov,
M. Andreotti,
D. Andreou,
D. Ao,
F. Archilli,
A. Artamonov,
M. Artuso,
E. Aslanides,
M. Atzeni,
B. Audurier,
I. Bachiller Perea,
S. Bachmann,
M. Bachmayer,
J.J. Back,
A. Bailly-reyre,
P. Baladron Rodriguez,
V. Balagura,
W. Baldini,
J. Baptista de Souza Leite,
M. Barbetti,
I. R. Barbosa,
R.J. Barlow,
S. Barsuk,
W. Barter,
M. Bartolini,
F. Baryshnikov,
J.M. Basels,
G. Bassi,
B. Batsukh,
A. Battig,
A. Bay,
A. Beck,
M. Becker,
F. Bedeschi,
I.B. Bediaga,
A. Beiter,
S. Belin,
V. Bellee,
K. Belous,
I. Belov,
I. Belyaev,
G. Benane,
G. Bencivenni,
E. Ben-Haim,
A. Berezhnoy,
R. Bernet,
S. Bernet Andres,
D. Berninghoff,
H.C. Bernstein,
C. Bertella,
A. Bertolin,
C. Betancourt,
F. Betti,
Ia. Bezshyiko,
J. Bhom,
L. Bian,
M.S. Bieker,
N.V. Biesuz,
P. Billoir,
A. Biolchini,
M. Birch,
F.C.R. Bishop,
A. Bitadze,
A. Bizzeti,
M.P. Blago,
T. Blake,
F. Blanc,
J.E. Blank,
S. Blusk,
D. Bobulska,
V. Bocharnikov,
J.A. Boelhauve,
O. Boente Garcia,
T. Boettcher,
A. Boldyrev,
C.S. Bolognani,
R. Bolzonella,
N. Bondar,
F. Borgato,
S. Borghi,
M. Borsato,
J.T. Borsuk,
S.A. Bouchiba,
T.J.V. Bowcock,
A. Boyer,
C. Bozzi,
M.J. Bradley,
S. Braun,
A. Brea Rodriguez,
N. Breer,
J. Brodzicka,
A. Brossa Gonzalo,
J. Brown,
D. Brundu,
A. Buonaura,
L. Buonincontri,
A.T. Burke,
C. Burr,
A. Bursche,
A. Butkevich,
J.S. Butter,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
R. Calabrese,
L. Calefice,
S. Cali,
M. Calvi,
M. Calvo Gomez,
P. Campana,
D.H. Campora Perez,
A.F. Campoverde Quezada,
S. Capelli,
L. Capriotti,
A. Carbone,
R. Cardinale,
A. Cardini,
P. Carniti,
L. Carus,
A. Casais Vidal,
R. Caspary,
G. Casse,
M. Cattaneo,
G. Cavallero,
V. Cavallini,
S. Celani,
J. Cerasoli,
D. Cervenkov,
A.J. Chadwick,
I. Chahrour,
M.G. Chapman,
M. Charles,
Ph. Charpentier,
C.A. Chavez Barajas,
M. Chefdeville,
C. Chen,
S. Chen,
A. Chernov,
S. Chernyshenko,
V. Chobanova,
S. Cholak,
M. Chrzaszcz,
A. Chubykin,
V. Chulikov,
P. Ciambrone,
M.F. Cicala,
X. Cid Vidal,
G. Ciezarek,
P. Cifra,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
J.L. Cobbledick,
V. Coco,
J. Cogan,
E. Cogneras,
L. Cojocariu,
P. Collins,
T. Colombo,
A. Comerma-Montells,
L. Congedo,
A. Contu,
N. Cooke,
I. Corredoira ,
G. Corti,
B. Couturier,
D.C. Craik,
M. Cruz Torres,
R. Currie,
C.L. Da Silva,
S. Dadabaev,
L. Dai,
X. Dai,
E. Dall'Occo,
J. Dalseno,
C. D'Ambrosio,
J. Daniel,
A. Danilina,
P. d'Argent,
J.E. Davies,
A. Davis,
O. De Aguiar Francisco,
J. de Boer,
K. De Bruyn,
S. De Capua,
M. De Cian,
U. De Freitas Carneiro Da Graca,
E. De Lucia,
J.M. De Miranda,
L. De Paula,
M. De Serio,
D. De Simone,
P. De Simone,
F. De Vellis,
J.A. de Vries,
C.T. Dean,
F. Debernardis,
D. Decamp,
V. Dedu,
L. Del Buono,
B. Delaney,
H.-P. Dembinski,
V. Denysenko,
O. Deschamps,
F. Dettori,
B. Dey,
P. Di Nezza,
I. Diachkov,
S. Didenko,
S. Ding,
V. Dobishuk,
A. Dolmatov,
C. Dong,
A.M. Donohoe,
F. Dordei,
A.C. dos Reis,
L. Douglas,
A.G. Downes,
P. Duda,
M.W. Dudek,
L. Dufour,
V. Duk,
P. Durante,
M. M. Duras,
J.M. Durham,
D. Dutta,
A. Dziurda,
A. Dzyuba,
S. Easo,
U. Egede,
A. Egorychev,
V. Egorychev,
C. Eirea Orro,
S. Eisenhardt,
E. Ejopu,
S. Ek-In,
L. Eklund,
M. Elashri,
J. Ellbracht,
S. Ely,
A. Ene,
E. Epple,
S. Escher,
J. Eschle,
S. Esen,
T. Evans,
F. Fabiano,
L.N. Falcao,
Y. Fan,
B. Fang,
L. Fantini,
M. Faria,
S. Farry,
D. Fazzini,
L. Felkowski,
M. Feng,
M. Feo,
M. Fernandez Gomez,
A.D. Fernez,
F. Ferrari,
L. Ferreira Lopes,
F. Ferreira Rodrigues,
S. Ferreres Sole,
M. Ferrillo,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiorini,
M. Firlej,
K.M. Fischer,
D.S. Fitzgerald,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
M. Fontana,
F. Fontanelli,
R. Forty,
D. Foulds-Holt,
V. Franco Lima,
M. Franco Sevilla,
M. Frank,
E. Franzoso,
G. Frau,
C. Frei,
D.A. Friday,
L. Frontini,
J. Fu,
Q. Fuehring,
T. Fulghesu,
E. Gabriel,
G. Galati,
M.D. Galati,
A. Gallas Torreira,
D. Galli,
S. Gambetta,
M. Gandelman,
P. Gandini,
H. Gao,
R. Gao,
Y. Gao,
Y. Gao,
M. Garau,
L.M. Garcia Martin,
P. Garcia Moreno,
J. Garc{\'\i}a Pardi{\~n}as,
B. Garcia Plana,
F.A. Garcia Rosales,
L. Garrido,
C. Gaspar,
R.E. Geertsema,
L.L. Gerken,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
L. Giambastiani,
V. Gibson,
H.K. Giemza,
A.L. Gilman,
M. Giovannetti,
A. Giovent{\`u},
P. Gironella Gironell,
C. Giugliano,
M.A. Giza,
K. Gizdov,
E.L. Gkougkousis,
V.V. Gligorov,
C. G{\"o}bel,
E. Golobardes,
D. Golubkov,
A. Golutvin,
A. Gomes,
S. Gomez Fernandez,
F. Goncalves Abrantes,
M. Goncerz,
G. Gong,
I.V. Gorelov,
C. Gotti,
J.P. Grabowski,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
G. Graziani,
A. T. Grecu,
L.M. Greeven,
N.A. Grieser,
L. Grillo,
S. Gromov,
C.  Gu,
M. Guarise,
M. Guittiere,
V. Guliaeva,
P. A. G{\"u}nther,
A.K. Guseinov,
E. Gushchin,
Y. Guz,
T. Gys,
T. Hadavizadeh,
C. Hadjivasiliou,
G. Haefeli,
C. Haen,
J. Haimberger,
S.C. Haines,
T. Halewood-leagas,
M.M. Halvorsen,
P.M. Hamilton,
J. Hammerich,
Q. Han,
X. Han,
S. Hansmann-Menzemer,
L. Hao,
N. Harnew,
T. Harrison,
C. Hasse,
M. Hatch,
J. He,
K. Heijhoff,
F. Hemmer,
C. Henderson,
R.D.L. Henderson,
A.M. Hennequin,
K. Hennessy,
L. Henry,
J. Herd,
J. Heuel,
A. Hicheur,
D. Hill,
M. Hilton,
S.E. Hollitt,
J. Horswill,
R. Hou,
Y. Hou,
J. Hu,
J. Hu,
W. Hu,
X. Hu,
W. Huang,
X. Huang,
W. Hulsbergen,
R.J. Hunter,
M. Hushchyn,
D. Hutchcroft,
P. Ibis,
M. Idzik,
D. Ilin,
P. Ilten,
A. Inglessi,
A. Iniukhin,
A. Ishteev,
K. Ivshin,
R. Jacobsson,
H. Jage,
S.J. Jaimes Elles,
S. Jakobsen,
E. Jans,
B.K. Jashal,
A. Jawahery,
V. Jevtic,
E. Jiang,
X. Jiang,
Y. Jiang,
M. John,
D. Johnson,
C.R. Jones,
T.P. Jones,
S. Joshi,
B. Jost,
N. Jurik,
I. Juszczak,
S. Kandybei,
Y. Kang,
M. Karacson,
D. Karpenkov,
M. Karpov,
J.W. Kautz,
F. Keizer,
D.M. Keller,
M. Kenzie,
T. Ketel,
B. Khanji,
A. Kharisova,
S. Kholodenko,
G. Khreich,
T. Kirn,
V.S. Kirsebom,
O. Kitouni,
S. Klaver,
N. Kleijne,
K. Klimaszewski,
M.R. Kmiec,
S. Koliiev,
L. Kolk,
A. Kondybayeva,
A. Konoplyannikov,
P. Kopciewicz,
R. Kopecna,
P. Koppenburg,
M. Korolev,
I. Kostiuk,
O. Kot,
S. Kotriakhova,
A. Kozachuk,
P. Kravchenko,
L. Kravchuk,
M. Kreps,
S. Kretzschmar,
P. Krokovny,
W. Krupa,
W. Krzemien,
J. Kubat,
S. Kubis,
W. Kucewicz,
M. Kucharczyk,
V. Kudryavtsev,
E. Kulikova,
A. Kupsc,
D. Lacarrere,
G. Lafferty,
A. Lai,
A. Lampis,
D. Lancierini,
C. Landesa Gomez,
J.J. Lane,
R. Lane,
C. Langenbruch,
J. Langer,
O. Lantwin,
T. Latham,
F. Lazzari,
C. Lazzeroni,
R. Le Gac,
S.H. Lee,
R. Lef{\`e}vre,
A. Leflat,
S. Legotin,
O. Leroy,
T. Lesiak,
B. Leverington,
A. Li,
H. Li,
K. Li,
P. Li,
P.-R. Li,
S. Li,
T. Li,
T. Li,
Y. Li,
Z. Li,
Z. Lian,
X. Liang,
C. Lin,
T. Lin,
R. Lindner,
V. Lisovskyi,
R. Litvinov,
G. Liu,
H. Liu,
K. Liu,
Q. Liu,
S. Liu,
A. Lobo Salvia,
A. Loi,
R. Lollini,
J. Lomba Castro,
I. Longstaff,
J.H. Lopes,
A. Lopez Huertas,
S. L{\'o}pez Soli{\~n}o,
G.H. Lovell,
Y. Lu,
C. Lucarelli,
D. Lucchesi,
S. Luchuk,
M. Lucio Martinez,
V. Lukashenko,
Y. Luo,
A. Lupato,
E. Luppi,
K. Lynch,
X.-R. Lyu,
R. Ma,
S. Maccolini,
F. Machefert,
F. Maciuc,
I. Mackay,
V. Macko,
L.R. Madhan Mohan,
A. Maevskiy,
D. Maisuzenko,
M.W. Majewski,
J.J. Malczewski,
S. Malde,
B. Malecki,
A. Malinin,
T. Maltsev,
G. Manca,
G. Mancinelli,
C. Mancuso,
R. Manera Escalero,
D. Manuzzi,
C.A. Manzari,
D. Marangotto,
J.F. Marchand,
U. Marconi,
S. Mariani,
C. Marin Benito,
J. Marks,
A.M. Marshall,
P.J. Marshall,
G. Martelli,
G. Martellotti,
L. Martinazzoli,
M. Martinelli,
D. Martinez Santos,
F. Martinez Vidal,
A. Massafferri,
M. Materok,
R. Matev,
A. Mathad,
V. Matiunin,
C. Matteuzzi,
K.R. Mattioli,
A. Mauri,
E. Maurice,
J. Mauricio,
M. Mazurek,
M. McCann,
L. Mcconnell,
T.H. McGrath,
N.T. McHugh,
A. McNab,
R. McNulty,
B. Meadows,
G. Meier,
D. Melnychuk,
S. Meloni,
M. Merk,
A. Merli,
L. Meyer Garcia,
D. Miao,
H. Miao,
M. Mikhasenko,
D.A. Milanes,
M. Milovanovic,
M.-N. Minard,
A. Minotti,
E. Minucci,
T. Miralles,
S.E. Mitchell,
B. Mitreska,
D.S. Mitzel,
A. Modak,
A. M{\"o}dden ,
R.A. Mohammed,
R.D. Moise,
S. Mokhnenko,
T. Momb{\"a}cher,
M. Monk,
I.A. Monroy,
S. Monteil,
G. Morello,
M.J. Morello,
M.P. Morgenthaler,
J. Moron,
A.B. Morris,
A.G. Morris,
R. Mountain,
H. Mu,
E. Muhammad,
F. Muheim,
M. Mulder,
K. M{\"u}ller,
D. Murray,
R. Murta,
P. Muzzetto,
P. Naik,
T. Nakada,
R. Nandakumar,
T. Nanut,
I. Nasteva,
M. Needham,
N. Neri,
S. Neubert,
N. Neufeld,
P. Neustroev,
R. Newcombe,
J. Nicolini,
D. Nicotra,
E.M. Niel,
S. Nieswand,
N. Nikitin,
N.S. Nolte,
C. Normand,
J. Novoa Fernandez,
G. Nowak,
C. Nunez,
A. Oblakowska-Mucha,
V. Obraztsov,
T. Oeser,
S. Okamura,
R. Oldeman,
F. Oliva,
M. Olocco,
C.J.G. Onderwater,
R.H. O'Neil,
J.M. Otalora Goicochea,
T. Ovsiannikova,
P. Owen,
A. Oyanguren,
O. Ozcelik,
K.O. Padeken,
B. Pagare,
P.R. Pais,
T. Pajero,
A. Palano,
M. Palutan,
G. Panshin,
L. Paolucci,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
C. Pappenheimer,
C. Parkes,
B. Passalacqua,
G. Passaleva,
A. Pastore,
M. Patel,
C. Patrignani,
C.J. Pawley,
A. Pellegrino,
M. Pepe Altarelli,
S. Perazzini,
D. Pereima,
A. Pereiro Castro,
P. Perret,
K. Petridis,
A. Petrolini,
S. Petrucci,
M. Petruzzo,
H. Pham,
A. Philippov,
R. Piandani,
L. Pica,
M. Piccini,
B. Pietrzyk,
G. Pietrzyk,
D. Pinci,
F. Pisani,
M. Pizzichemi,
V. Placinta,
J. Plews,
M. Plo Casasus,
F. Polci,
M. Poli Lener,
A. Poluektov,
N. Polukhina,
I. Polyakov,
E. Polycarpo,
S. Ponce,
D. Popov,
S. Poslavskii,
K. Prasanth,
L. Promberger,
C. Prouve,
V. Pugatch,
V. Puill,
G. Punzi,
H.R. Qi,
W. Qian,
N. Qin,
S. Qu,
R. Quagliani,
B. Rachwal,
J.H. Rademacker,
R. Rajagopalan,
M. Rama,
M. Ramos Pernas,
M.S. Rangel,
F. Ratnikov,
G. Raven,
M. Rebollo De Miguel,
F. Redi,
J. Reich,
F. Reiss,
Z. Ren,
P.K. Resmi,
R. Ribatti,
A.M. Ricci,
S. Ricciardi,
K. Richardson,
M. Richardson-Slipper,
K. Rinnert,
P. Robbe,
G. Robertson,
E. Rodrigues,
E. Rodriguez Fernandez,
J.A. Rodriguez Lopez,
E. Rodriguez Rodriguez,
D.L. Rolf,
A. Rollings,
P. Roloff,
V. Romanovskiy,
M. Romero Lamas,
A. Romero Vidal,
M. Rotondo,
M.S. Rudolph,
T. Ruf,
R.A. Ruiz Fernandez,
J. Ruiz Vidal,
A. Ryzhikov,
J. Ryzka,
J.J. Saborido Silva,
N. Sagidova,
N. Sahoo,
B. Saitta,
M. Salomoni,
C. Sanchez Gras,
I. Sanderswood,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
L. Santoro ,
E. Santovetti,
D. Saranin,
G. Sarpis,
M. Sarpis,
A. Sarti,
C. Satriano,
A. Satta,
M. Saur,
D. Savrina,
H. Sazak,
L.G. Scantlebury Smead,
A. Scarabotto,
S. Schael,
S. Scherl,
A. M.  Schertz,
M. Schiller,
H. Schindler,
M. Schmelling,
B. Schmidt,
S. Schmitt,
O. Schneider,
A. Schopper,
M. Schubiger,
N. Schulte,
S. Schulte,
M.H. Schune,
R. Schwemmer,
G. Schwering,
B. Sciascia,
A. Sciuccati,
S. Sellam,
A. Semennikov,
M. Senghi Soares,
A. Sergi,
N. Serra,
L. Sestini,
A. Seuthe,
Y. Shang,
D.M. Shangase,
M. Shapkin,
I. Shchemerov,
L. Shchutska,
T. Shears,
L. Shekhtman,
Z. Shen,
S. Sheng,
V. Shevchenko,
B. Shi,
E.B. Shields,
Y. Shimizu,
E. Shmanin,
R. Shorkin,
J.D. Shupperd,
B.G. Siddi,
R. Silva Coutinho,
G. Simi,
S. Simone,
M. Singla,
N. Skidmore,
R. Skuza,
T. Skwarnicki,
M.W. Slater,
J.C. Smallwood,
J.G. Smeaton,
E. Smith,
K. Smith,
M. Smith,
A. Snoch,
L. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
A. Solomin,
A. Solovev,
I. Solovyev,
R. Song,
Y. Song,
F.L. Souza De Almeida,
B. Souza De Paula,
E. Spadaro Norella,
E. Spedicato,
J.G. Speer,
E. Spiridenkov,
P. Spradlin,
V. Sriskaran,
F. Stagni,
M. Stahl,
S. Stahl,
S. Stanislaus,
E.N. Stein,
O. Steinkamp,
O. Stenyakin,
H. Stevens,
D. Strekalina,
Y. Su,
F. Suljik,
J. Sun,
L. Sun,
Y. Sun,
P.N. Swallow,
K. Swientek,
A. Szabelski,
T. Szumlak,
M. Szymanski,
Y. Tan,
S. Taneja,
M.D. Tat,
A. Terentev,
F. Teubert,
E. Thomas,
D.J.D. Thompson,
H. Tilquin,
V. Tisserand,
S. T'Jampens,
M. Tobin,
L. Tomassetti,
G. Tonani,
X. Tong,
D. Torres Machado,
L. Toscano,
D.Y. Tou,
C. Trippl,
G. Tuci,
N. Tuning,
A. Ukleja,
D.J. Unverzagt,
E. Ursov,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
V. Vagnoni,
A. Valassi,
G. Valenti,
N. Valls Canudas,
M. Van Dijk,
H. Van Hecke,
E. van Herwijnen,
C.B. Van Hulse,
M. van Veghel,
R. Vazquez Gomez,
P. Vazquez Regueiro,
C. V{\'a}zquez Sierra,
S. Vecchi,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Vesterinen,
D.  Vieira,
M. Vieites Diaz,
X. Vilasis-Cardona,
E. Vilella Figueras,
A. Villa,
P. Vincent,
F.C. Volle,
D. vom Bruch,
V. Vorobyev,
N. Voropaev,
K. Vos,
C. Vrahas,
J. Walsh,
E.J. Walton,
G. Wan,
C. Wang,
G. Wang,
J. Wang,
J. Wang,
J. Wang,
J. Wang,
M. Wang,
R. Wang,
X. Wang,
Y. Wang,
Z. Wang,
Z. Wang,
Z. Wang,
J.A. Ward,
N.K. Watson,
D. Websdale,
Y. Wei,
B.D.C. Westhenry,
D.J. White,
M. Whitehead,
A.R. Wiederhold,
D. Wiedner,
G. Wilkinson,
M.K. Wilkinson,
I. Williams,
M. Williams,
M.R.J. Williams,
R. Williams,
F.F. Wilson,
W. Wislicki,
M. Witek,
L. Witola,
C.P. Wong,
G. Wormser,
S.A. Wotton,
H. Wu,
J. Wu,
Y. Wu,
K. Wyllie,
Z. Xiang,
Y. Xie,
A. Xu,
J. Xu,
L. Xu,
L. Xu,
M. Xu,
Q. Xu,
Z. Xu,
Z. Xu,
Z. Xu,
D. Yang,
S. Yang,
X. Yang,
Y. Yang,
Z. Yang,
Z. Yang,
V. Yeroshenko,
H. Yeung,
H. Yin,
J. Yu,
X. Yuan,
E. Zaffaroni,
M. Zavertyaev,
M. Zdybal,
M. Zeng,
C. Zhang,
D. Zhang,
J. Zhang,
L. Zhang,
S. Zhang,
S. Zhang,
Y. Zhang,
Y. Zhang,
Y. Zhao,
A. Zharkova,
A. Zhelezov,
Y. Zheng,
T. Zhou,
X. Zhou,
Y. Zhou,
V. Zhovkovska,
L. Z.  Zhu,
X. Zhu,
X. Zhu,
Z. Zhu,
V. Zhukov,
J. Zhuo,
Q. Zou,
S. Zucchelli,
D. Zuliani,
G. Zunica

==> LHCb_authorlist.tex <==
% $Id: LHCb_authorlist.tex 78711 2015-08-06 07:54:32Z apuignav $
% ===============================================================================
% Purpose: example of authorlist for LHCb template
% Author:
% Created on: 2009-09-24
% ===============================================================================

%\documentclass[a4paper]{article}
%\setlength{\oddsidemargin}{0cm}
%\setlength{\evensidemargin}{0cm}
%\setlength{\textwidth}{16.5cm}
%\setlength{\parindent}{0cm}
%\begin{document}
\centerline{\large\normalfont\bfseries LHCb collaboration}
\begin{flushleft}
\small
%-- LHCb Authorlist, Example typesetting
%-- 
A.~N.~Other$^{1}$.\bigskip\newline{\it
\footnotesize
$ ^{1}$University of nowhere\\
}
%-- 
%-- 
\end{flushleft}
%\end{document}


==> acknowledgements_full.tex <==
\section*{Acknowledgements}
%
% These Acknowledgements valid from 3-May-2019
%
\noindent We express our gratitude to our colleagues in the CERN
accelerator departments for the excellent performance of the LHC. We
thank the technical and administrative staff at the LHCb
institutes.
We acknowledge support from CERN and from the national agencies:
CAPES, CNPq, FAPERJ and FINEP (Brazil); 
MOST and NSFC (China); 
CNRS/IN2P3 (France); 
BMBF, DFG and MPG (Germany); 
INFN (Italy); 
NWO (Netherlands); 
MNiSW and NCN (Poland); 
MEN/IFA (Romania); 
MSHE (Russia); 
MICINN (Spain); 
SNSF and SER (Switzerland); 
NASU (Ukraine); 
STFC (United Kingdom); 
DOE NP and NSF (USA).
We acknowledge the computing resources that are provided by CERN, IN2P3
(France), KIT and DESY (Germany), INFN (Italy), SURF (Netherlands),
PIC (Spain), GridPP (United Kingdom), RRCKI and Yandex
LLC (Russia), CSCS (Switzerland), IFIN-HH (Romania), CBPF (Brazil),
PL-GRID (Poland) and NERSC (USA).
We are indebted to the communities behind the multiple open-source
software packages on which we depend.
Individual groups or members have received support from
ARC and ARDC (Australia);
Minciencias (Colombia);
AvH Foundation (Germany);
EPLANET, Marie Sk\l{}odowska-Curie Actions and ERC (European Union);
A*MIDEX, ANR, IPhU and Labex P2IO, and R\'{e}gion Auvergne-Rh\^{o}ne-Alpes (France);
Key Research Program of Frontier Sciences of CAS, CAS PIFI, CAS CCEPP, 
Fundamental Research Funds for the Central Universities, 
and Sci. \& Tech. Program of Guangzhou (China);
%Key Research Program of Frontier Sciences of CAS, CAS PIFI,
%Thousand Talents Program, and Sci. \& Tech. Program of Guangzhou (China);
RFBR, RSF and Yandex LLC (Russia);
GVA, XuntaGal and GENCAT (Spain);
SRC (Sweden);
the Leverhulme Trust, the Royal Society
 and UKRI (United Kingdom).



==> acknowledgements_intro.tex <==
\section{Acknowledgements paragraph}

Include the following text in the Acknowledgements section in all paper
drafts. It is not needed for analysis notes or conference reports.

The text below are the acknowledgements as approved by the collaboration
board. Extending the acknowledgements to include individuals from outside the
collaboration who have contributed to the analysis should be approved by the
EB. The extra acknowledgements are normally placed before the standard 
acknowledgements, unless it matches better with the text of the standard 
acknowledgements to put them elsewhere. They should be included in the draft 
for the first circulation. Except in exceptional circumstances, to be approved by the
EB chair, authors of the paper should not be named in extended acknowledgements.

%\vspace{1cm}

\input{acknowledgements}


==> lhcb-symbols-list.tex <==
% This is an automatically generated appendix to template.tex. 
% When included it will show all the symbols defined in lhcb-symbols-def.tex.
%
% To regenerate with the latest definitions run the script ./listsymbols

\section{List of all symbols}
\label{sec:listofsymbols}
\subsection{Experiments}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash lhcb} & \lhcb & \texttt{\textbackslash atlas} & \atlas & \texttt{\textbackslash cms} & \cms \\
\texttt{\textbackslash alice} & \alice & \texttt{\textbackslash babar} & \babar & \texttt{\textbackslash belle} & \belle \\
\texttt{\textbackslash cleo} & \cleo & \texttt{\textbackslash cdf} & \cdf & \texttt{\textbackslash dzero} & \dzero \\
\texttt{\textbackslash aleph} & \aleph & \texttt{\textbackslash delphi} & \delphi & \texttt{\textbackslash opal} & \opal \\
\texttt{\textbackslash lthree} & \lthree & \texttt{\textbackslash sld} & \sld & \texttt{\textbackslash cern} & \cern \\
\texttt{\textbackslash lhc} & \lhc & \texttt{\textbackslash lep} & \lep & \texttt{\textbackslash tevatron} & \tevatron \\
\end{tabular*}

\subsubsection{LHCb sub-detectors and sub-systems}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash velo} & \velo & \texttt{\textbackslash rich} & \rich & \texttt{\textbackslash richone} & \richone \\
\texttt{\textbackslash richtwo} & \richtwo & \texttt{\textbackslash ttracker} & \ttracker & \texttt{\textbackslash intr} & \intr \\
\texttt{\textbackslash st} & \st & \texttt{\textbackslash ot} & \ot & \texttt{\textbackslash herschel} & \herschel \\
\texttt{\textbackslash spd} & \spd & \texttt{\textbackslash presh} & \presh & \texttt{\textbackslash ecal} & \ecal \\
\texttt{\textbackslash hcal} & \hcal & \texttt{\textbackslash MagUp} & \MagUp & \texttt{\textbackslash MagDown} & \MagDown \\
\texttt{\textbackslash ode} & \ode & \texttt{\textbackslash daq} & \daq & \texttt{\textbackslash tfc} & \tfc \\
\texttt{\textbackslash ecs} & \ecs & \texttt{\textbackslash lone} & \lone & \texttt{\textbackslash hlt} & \hlt \\
\texttt{\textbackslash hltone} & \hltone & \texttt{\textbackslash hlttwo} & \hlttwo &  \\
\end{tabular*}

\subsection{Particles}
\subsubsection{Leptons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash electron} & \electron & \texttt{\textbackslash en} & \en & \texttt{\textbackslash ep} & \ep \\
\texttt{\textbackslash epm} & \epm & \texttt{\textbackslash epem} & \epem & \texttt{\textbackslash muon} & \muon \\
\texttt{\textbackslash mup} & \mup & \texttt{\textbackslash mun} & \mun & \texttt{\textbackslash mumu} & \mumu \\
\texttt{\textbackslash tauon} & \tauon & \texttt{\textbackslash taup} & \taup & \texttt{\textbackslash taum} & \taum \\
\texttt{\textbackslash tautau} & \tautau & \texttt{\textbackslash lepton} & \lepton & \texttt{\textbackslash ellm} & \ellm \\
\texttt{\textbackslash ellp} & \ellp & \texttt{\textbackslash ellell} & \ellell & \texttt{\textbackslash neu} & \neu \\
\texttt{\textbackslash neub} & \neub & \texttt{\textbackslash neue} & \neue & \texttt{\textbackslash neueb} & \neueb \\
\texttt{\textbackslash neum} & \neum & \texttt{\textbackslash neumb} & \neumb & \texttt{\textbackslash neut} & \neut \\
\texttt{\textbackslash neutb} & \neutb & \texttt{\textbackslash neul} & \neul & \texttt{\textbackslash neulb} & \neulb \\
\end{tabular*}

\subsubsection{Gauge bosons and scalars}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash g} & \g & \texttt{\textbackslash H} & \H & \texttt{\textbackslash Hp} & \Hp \\
\texttt{\textbackslash Hm} & \Hm & \texttt{\textbackslash Hpm} & \Hpm & \texttt{\textbackslash W} & \W \\
\texttt{\textbackslash Wp} & \Wp & \texttt{\textbackslash Wm} & \Wm & \texttt{\textbackslash Wpm} & \Wpm \\
\texttt{\textbackslash Z} & \Z &  \\
\end{tabular*}

\subsubsection{Quarks}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash quark} & \quark & \texttt{\textbackslash quarkbar} & \quarkbar & \texttt{\textbackslash qqbar} & \qqbar \\
\texttt{\textbackslash uquark} & \uquark & \texttt{\textbackslash uquarkbar} & \uquarkbar & \texttt{\textbackslash uubar} & \uubar \\
\texttt{\textbackslash dquark} & \dquark & \texttt{\textbackslash dquarkbar} & \dquarkbar & \texttt{\textbackslash ddbar} & \ddbar \\
\texttt{\textbackslash squark} & \squark & \texttt{\textbackslash squarkbar} & \squarkbar & \texttt{\textbackslash ssbar} & \ssbar \\
\texttt{\textbackslash cquark} & \cquark & \texttt{\textbackslash cquarkbar} & \cquarkbar & \texttt{\textbackslash ccbar} & \ccbar \\
\texttt{\textbackslash bquark} & \bquark & \texttt{\textbackslash bquarkbar} & \bquarkbar & \texttt{\textbackslash bbbar} & \bbbar \\
\texttt{\textbackslash tquark} & \tquark & \texttt{\textbackslash tquarkbar} & \tquarkbar & \texttt{\textbackslash ttbar} & \ttbar \\
\end{tabular*}

\subsubsection{Light mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash hadron} & \hadron & \texttt{\textbackslash pion} & \pion & \texttt{\textbackslash piz} & \piz \\
\texttt{\textbackslash pizs} & \pizs & \texttt{\textbackslash pip} & \pip & \texttt{\textbackslash pim} & \pim \\
\texttt{\textbackslash pipm} & \pipm & \texttt{\textbackslash pimp} & \pimp & \texttt{\textbackslash rhomeson} & \rhomeson \\
\texttt{\textbackslash rhoz} & \rhoz & \texttt{\textbackslash rhop} & \rhop & \texttt{\textbackslash rhom} & \rhom \\
\texttt{\textbackslash rhopm} & \rhopm & \texttt{\textbackslash rhomp} & \rhomp & \texttt{\textbackslash kaon} & \kaon \\
\texttt{\textbackslash Kb} & \Kb & \texttt{\textbackslash KorKbar} & \KorKbar & \texttt{\textbackslash Kz} & \Kz \\
\texttt{\textbackslash Kzb} & \Kzb & \texttt{\textbackslash Kp} & \Kp & \texttt{\textbackslash Km} & \Km \\
\texttt{\textbackslash Kpm} & \Kpm & \texttt{\textbackslash Kmp} & \Kmp & \texttt{\textbackslash KS} & \KS \\
\texttt{\textbackslash KL} & \KL & \texttt{\textbackslash Kstarz} & \Kstarz & \texttt{\textbackslash Kstarzb} & \Kstarzb \\
\texttt{\textbackslash Kstar} & \Kstar & \texttt{\textbackslash Kstarb} & \Kstarb & \texttt{\textbackslash Kstarp} & \Kstarp \\
\texttt{\textbackslash Kstarm} & \Kstarm & \texttt{\textbackslash Kstarpm} & \Kstarpm & \texttt{\textbackslash Kstarmp} & \Kstarmp \\
\texttt{\textbackslash etaz} & \etaz & \texttt{\textbackslash etapr} & \etapr & \texttt{\textbackslash phiz} & \phiz \\
\texttt{\textbackslash omegaz} & \omegaz &  \\
\end{tabular*}

\subsubsection{Heavy mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash D} & \D & \texttt{\textbackslash Db} & \Db & \texttt{\textbackslash DorDbar} & \DorDbar \\
\texttt{\textbackslash Dz} & \Dz & \texttt{\textbackslash Dzb} & \Dzb & \texttt{\textbackslash Dp} & \Dp \\
\texttt{\textbackslash Dm} & \Dm & \texttt{\textbackslash Dpm} & \Dpm & \texttt{\textbackslash Dmp} & \Dmp \\
\texttt{\textbackslash Dstar} & \Dstar & \texttt{\textbackslash Dstarb} & \Dstarb & \texttt{\textbackslash Dstarz} & \Dstarz \\
\texttt{\textbackslash Dstarzb} & \Dstarzb & \texttt{\textbackslash Dstarp} & \Dstarp & \texttt{\textbackslash Dstarm} & \Dstarm \\
\texttt{\textbackslash Dstarpm} & \Dstarpm & \texttt{\textbackslash Dstarmp} & \Dstarmp & \texttt{\textbackslash Ds} & \Ds \\
\texttt{\textbackslash Dsp} & \Dsp & \texttt{\textbackslash Dsm} & \Dsm & \texttt{\textbackslash Dspm} & \Dspm \\
\texttt{\textbackslash Dsmp} & \Dsmp & \texttt{\textbackslash Dss} & \Dss & \texttt{\textbackslash Dssp} & \Dssp \\
\texttt{\textbackslash Dssm} & \Dssm & \texttt{\textbackslash Dsspm} & \Dsspm & \texttt{\textbackslash Dssmp} & \Dssmp \\
\texttt{\textbackslash B} & \B & \texttt{\textbackslash Bbar} & \Bbar & \texttt{\textbackslash Bb} & \Bb \\
\texttt{\textbackslash BorBbar} & \BorBbar & \texttt{\textbackslash Bz} & \Bz & \texttt{\textbackslash Bzb} & \Bzb \\
\texttt{\textbackslash Bu} & \Bu & \texttt{\textbackslash Bub} & \Bub & \texttt{\textbackslash Bp} & \Bp \\
\texttt{\textbackslash Bm} & \Bm & \texttt{\textbackslash Bpm} & \Bpm & \texttt{\textbackslash Bmp} & \Bmp \\
\texttt{\textbackslash Bd} & \Bd & \texttt{\textbackslash Bs} & \Bs & \texttt{\textbackslash Bsb} & \Bsb \\
\texttt{\textbackslash Bdb} & \Bdb & \texttt{\textbackslash Bc} & \Bc & \texttt{\textbackslash Bcp} & \Bcp \\
\texttt{\textbackslash Bcm} & \Bcm & \texttt{\textbackslash Bcpm} & \Bcpm &  \\
\end{tabular*}

\subsubsection{Onia}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash jpsi} & \jpsi & \texttt{\textbackslash psitwos} & \psitwos & \texttt{\textbackslash psiprpr} & \psiprpr \\
\texttt{\textbackslash etac} & \etac & \texttt{\textbackslash chiczero} & \chiczero & \texttt{\textbackslash chicone} & \chicone \\
\texttt{\textbackslash chictwo} & \chictwo & \texttt{\textbackslash OneS} & \OneS & \texttt{\textbackslash TwoS} & \TwoS \\
\texttt{\textbackslash ThreeS} & \ThreeS & \texttt{\textbackslash FourS} & \FourS & \texttt{\textbackslash FiveS} & \FiveS \\
\texttt{\textbackslash chic} & \chic &  \\
\end{tabular*}

\subsubsection{Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash proton} & \proton & \texttt{\textbackslash antiproton} & \antiproton & \texttt{\textbackslash neutron} & \neutron \\
\texttt{\textbackslash antineutron} & \antineutron & \texttt{\textbackslash Deltares} & \Deltares & \texttt{\textbackslash Deltaresbar} & \Deltaresbar \\
\texttt{\textbackslash Xires} & \Xires & \texttt{\textbackslash Xiresbar} & \Xiresbar & \texttt{\textbackslash Lz} & \Lz \\
\texttt{\textbackslash Lbar} & \Lbar & \texttt{\textbackslash LorLbar} & \LorLbar & \texttt{\textbackslash Lambdares} & \Lambdares \\
\texttt{\textbackslash Lambdaresbar} & \Lambdaresbar & \texttt{\textbackslash Sigmares} & \Sigmares & \texttt{\textbackslash Sigmaresbar} & \Sigmaresbar \\
\texttt{\textbackslash Sigmaresbarz} & \Sigmaresbarz & \texttt{\textbackslash Omegares} & \Omegares & \texttt{\textbackslash Omegaresbar} & \Omegaresbar \\
\texttt{\textbackslash Lb} & \Lb & \texttt{\textbackslash Lbbar} & \Lbbar & \texttt{\textbackslash Lc} & \Lc \\
\texttt{\textbackslash Lcbar} & \Lcbar & \texttt{\textbackslash Xib} & \Xib & \texttt{\textbackslash Xibz} & \Xibz \\
\texttt{\textbackslash Xibm} & \Xibm & \texttt{\textbackslash Xibbar} & \Xibbar & \texttt{\textbackslash Xibbarz} & \Xibbarz \\
\texttt{\textbackslash Xibbarp} & \Xibbarp & \texttt{\textbackslash Xic} & \Xic & \texttt{\textbackslash Xicz} & \Xicz \\
\texttt{\textbackslash Xicp} & \Xicp & \texttt{\textbackslash Xicbar} & \Xicbar & \texttt{\textbackslash Xicbarz} & \Xicbarz \\
\texttt{\textbackslash Xicbarm} & \Xicbarm & \texttt{\textbackslash Omegac} & \Omegac & \texttt{\textbackslash Omegacbar} & \Omegacbar \\
\texttt{\textbackslash Omegab} & \Omegab & \texttt{\textbackslash Omegabbar} & \Omegabbar &  \\
\end{tabular*}

\subsection{Physics symbols}
\subsubsection{Decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BF} & \BF & \texttt{\textbackslash BRvis} & \BRvis & \texttt{\textbackslash BR} & \BR \\
\texttt{\textbackslash decay[2] \textbackslash decay\{\Pa\}\{\Pb \Pc\}} & \decay{\Pa}{\Pb \Pc} & \texttt{\textbackslash ra} & \ra & \texttt{\textbackslash to} & \to \\
\end{tabular*}

\subsubsection{Lifetimes}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tauBs} & \tauBs & \texttt{\textbackslash tauBd} & \tauBd & \texttt{\textbackslash tauBz} & \tauBz \\
\texttt{\textbackslash tauBu} & \tauBu & \texttt{\textbackslash tauDp} & \tauDp & \texttt{\textbackslash tauDz} & \tauDz \\
\texttt{\textbackslash tauL} & \tauL & \texttt{\textbackslash tauH} & \tauH &  \\
\end{tabular*}

\subsubsection{Masses}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash mBd} & \mBd & \texttt{\textbackslash mBp} & \mBp & \texttt{\textbackslash mBs} & \mBs \\
\texttt{\textbackslash mBc} & \mBc & \texttt{\textbackslash mLb} & \mLb &  \\
\end{tabular*}

\subsubsection{EW theory, groups}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash grpsuthree} & \grpsuthree & \texttt{\textbackslash grpsutw} & \grpsutw & \texttt{\textbackslash grpuone} & \grpuone \\
\texttt{\textbackslash ssqtw} & \ssqtw & \texttt{\textbackslash csqtw} & \csqtw & \texttt{\textbackslash stw} & \stw \\
\texttt{\textbackslash ctw} & \ctw & \texttt{\textbackslash ssqtwef} & \ssqtwef & \texttt{\textbackslash csqtwef} & \csqtwef \\
\texttt{\textbackslash stwef} & \stwef & \texttt{\textbackslash ctwef} & \ctwef & \texttt{\textbackslash gv} & \gv \\
\texttt{\textbackslash ga} & \ga & \texttt{\textbackslash order} & \order & \texttt{\textbackslash ordalph} & \ordalph \\
\texttt{\textbackslash ordalsq} & \ordalsq & \texttt{\textbackslash ordalcb} & \ordalcb &  \\
\end{tabular*}

\subsubsection{QCD parameters}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash as} & \as & \texttt{\textbackslash MSb} & \MSb & \texttt{\textbackslash lqcd} & \lqcd \\
\texttt{\textbackslash qsq} & \qsq &  \\
\end{tabular*}

\subsubsection{CKM, CP violation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eps} & \eps & \texttt{\textbackslash epsK} & \epsK & \texttt{\textbackslash epsB} & \epsB \\
\texttt{\textbackslash epsp} & \epsp & \texttt{\textbackslash CP} & \CP & \texttt{\textbackslash CPT} & \CPT \\
\texttt{\textbackslash rhobar} & \rhobar & \texttt{\textbackslash etabar} & \etabar & \texttt{\textbackslash Vud} & \Vud \\
\texttt{\textbackslash Vcd} & \Vcd & \texttt{\textbackslash Vtd} & \Vtd & \texttt{\textbackslash Vus} & \Vus \\
\texttt{\textbackslash Vcs} & \Vcs & \texttt{\textbackslash Vts} & \Vts & \texttt{\textbackslash Vub} & \Vub \\
\texttt{\textbackslash Vcb} & \Vcb & \texttt{\textbackslash Vtb} & \Vtb & \texttt{\textbackslash Vuds} & \Vuds \\
\texttt{\textbackslash Vcds} & \Vcds & \texttt{\textbackslash Vtds} & \Vtds & \texttt{\textbackslash Vuss} & \Vuss \\
\texttt{\textbackslash Vcss} & \Vcss & \texttt{\textbackslash Vtss} & \Vtss & \texttt{\textbackslash Vubs} & \Vubs \\
\texttt{\textbackslash Vcbs} & \Vcbs & \texttt{\textbackslash Vtbs} & \Vtbs &  \\
\end{tabular*}

\subsubsection{Oscillations}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dm} & \dm & \texttt{\textbackslash dms} & \dms & \texttt{\textbackslash dmd} & \dmd \\
\texttt{\textbackslash DG} & \DG & \texttt{\textbackslash DGs} & \DGs & \texttt{\textbackslash DGd} & \DGd \\
\texttt{\textbackslash Gs} & \Gs & \texttt{\textbackslash Gd} & \Gd & \texttt{\textbackslash MBq} & \MBq \\
\texttt{\textbackslash DGq} & \DGq & \texttt{\textbackslash Gq} & \Gq & \texttt{\textbackslash dmq} & \dmq \\
\texttt{\textbackslash GL} & \GL & \texttt{\textbackslash GH} & \GH & \texttt{\textbackslash DGsGs} & \DGsGs \\
\texttt{\textbackslash Delm} & \Delm & \texttt{\textbackslash ACP} & \ACP & \texttt{\textbackslash Adir} & \Adir \\
\texttt{\textbackslash Amix} & \Amix & \texttt{\textbackslash ADelta} & \ADelta & \texttt{\textbackslash phid} & \phid \\
\texttt{\textbackslash sinphid} & \sinphid & \texttt{\textbackslash phis} & \phis & \texttt{\textbackslash betas} & \betas \\
\texttt{\textbackslash sbetas} & \sbetas & \texttt{\textbackslash stbetas} & \stbetas & \texttt{\textbackslash stphis} & \stphis \\
\texttt{\textbackslash sinphis} & \sinphis &  \\
\end{tabular*}

\subsubsection{Tagging}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash edet} & \edet & \texttt{\textbackslash erec} & \erec & \texttt{\textbackslash esel} & \esel \\
\texttt{\textbackslash etrg} & \etrg & \texttt{\textbackslash etot} & \etot & \texttt{\textbackslash mistag} & \mistag \\
\texttt{\textbackslash wcomb} & \wcomb & \texttt{\textbackslash etag} & \etag & \texttt{\textbackslash etagcomb} & \etagcomb \\
\texttt{\textbackslash effeff} & \effeff & \texttt{\textbackslash effeffcomb} & \effeffcomb & \texttt{\textbackslash efftag} & \efftag \\
\texttt{\textbackslash effD} & \effD & \texttt{\textbackslash etagprompt} & \etagprompt & \texttt{\textbackslash etagLL} & \etagLL \\
\end{tabular*}

\subsubsection{Key decay channels}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdToKstmm} & \BdToKstmm & \texttt{\textbackslash BdbToKstmm} & \BdbToKstmm & \texttt{\textbackslash BsToJPsiPhi} & \BsToJPsiPhi \\
\texttt{\textbackslash BdToJPsiKst} & \BdToJPsiKst & \texttt{\textbackslash BdbToJPsiKst} & \BdbToJPsiKst & \texttt{\textbackslash BsPhiGam} & \BsPhiGam \\
\texttt{\textbackslash BdKstGam} & \BdKstGam & \texttt{\textbackslash BTohh} & \BTohh & \texttt{\textbackslash BdTopipi} & \BdTopipi \\
\texttt{\textbackslash BdToKpi} & \BdToKpi & \texttt{\textbackslash BsToKK} & \BsToKK & \texttt{\textbackslash BsTopiK} & \BsTopiK \\
\end{tabular*}

\subsubsection{Rare decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdKstee} & \BdKstee & \texttt{\textbackslash BdbKstee} & \BdbKstee & \texttt{\textbackslash bsll} & \bsll \\
\texttt{\textbackslash AFB} & \AFB & \texttt{\textbackslash FL} & \FL & \texttt{\textbackslash AT\#1 \textbackslash AT2} & \AT2 \\
\texttt{\textbackslash btosgam} & \btosgam & \texttt{\textbackslash btodgam} & \btodgam & \texttt{\textbackslash Bsmm} & \Bsmm \\
\texttt{\textbackslash Bdmm} & \Bdmm & \texttt{\textbackslash ctl} & \ctl & \texttt{\textbackslash ctk} & \ctk \\
\end{tabular*}

\subsubsection{Wilson coefficients and operators}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash C\#1 \textbackslash C9} & \C9 & \texttt{\textbackslash Cp\#1 \textbackslash Cp7} & \Cp7 & \texttt{\textbackslash Ceff\#1 \textbackslash Ceff9  } & \Ceff9   \\
\texttt{\textbackslash Cpeff\#1 \textbackslash Cpeff7} & \Cpeff7 & \texttt{\textbackslash Ope\#1 \textbackslash Ope2} & \Ope2 & \texttt{\textbackslash Opep\#1 \textbackslash Opep7} & \Opep7 \\
\end{tabular*}

\subsubsection{Charm}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash xprime} & \xprime & \texttt{\textbackslash yprime} & \yprime & \texttt{\textbackslash ycp} & \ycp \\
\texttt{\textbackslash agamma} & \agamma & \texttt{\textbackslash dkpicf} & \dkpicf &  \\
\end{tabular*}

\subsubsection{QM}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bra[1] \textbackslash bra\{a\}} & \bra{a} & \texttt{\textbackslash ket[1] \textbackslash ket\{b\}} & \ket{b} & \texttt{\textbackslash braket[2] \textbackslash braket\{a\}\{b\}} & \braket{a}{b} \\
\end{tabular*}

\subsection{Units}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash unit[1] \textbackslash unit\{kg\}} & \unit{kg} &  \\
\end{tabular*}

\subsubsection{Energy and momentum}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tev} & \tev & \texttt{\textbackslash gev} & \gev & \texttt{\textbackslash mev} & \mev \\
\texttt{\textbackslash kev} & \kev & \texttt{\textbackslash ev} & \ev & \texttt{\textbackslash gevc} & \gevc \\
\texttt{\textbackslash mevc} & \mevc & \texttt{\textbackslash gevcc} & \gevcc & \texttt{\textbackslash gevgevcccc} & \gevgevcccc \\
\texttt{\textbackslash mevcc} & \mevcc &  \\
\end{tabular*}

\subsubsection{Distance and area}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash km} & \km & \texttt{\textbackslash m} & \m & \texttt{\textbackslash ma} & \ma \\
\texttt{\textbackslash cm} & \cm & \texttt{\textbackslash cma} & \cma & \texttt{\textbackslash mm} & \mm \\
\texttt{\textbackslash mma} & \mma & \texttt{\textbackslash mum} & \mum & \texttt{\textbackslash muma} & \muma \\
\texttt{\textbackslash nm} & \nm & \texttt{\textbackslash fm} & \fm & \texttt{\textbackslash barn} & \barn \\
\texttt{\textbackslash mbarn} & \mbarn & \texttt{\textbackslash mub} & \mub & \texttt{\textbackslash nb} & \nb \\
\texttt{\textbackslash invnb} & \invnb & \texttt{\textbackslash pb} & \pb & \texttt{\textbackslash invpb} & \invpb \\
\texttt{\textbackslash fb} & \fb & \texttt{\textbackslash invfb} & \invfb & \texttt{\textbackslash ab} & \ab \\
\texttt{\textbackslash invab} & \invab &  \\
\end{tabular*}

\subsubsection{Time }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sec} & \sec & \texttt{\textbackslash ms} & \ms & \texttt{\textbackslash mus} & \mus \\
\texttt{\textbackslash ns} & \ns & \texttt{\textbackslash ps} & \ps & \texttt{\textbackslash fs} & \fs \\
\texttt{\textbackslash mhz} & \mhz & \texttt{\textbackslash khz} & \khz & \texttt{\textbackslash hz} & \hz \\
\texttt{\textbackslash invps} & \invps & \texttt{\textbackslash invns} & \invns & \texttt{\textbackslash yr} & \yr \\
\texttt{\textbackslash hr} & \hr &  \\
\end{tabular*}

\subsubsection{Temperature}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degc} & \degc & \texttt{\textbackslash degk} & \degk &  \\
\end{tabular*}

\subsubsection{Material lengths, radiation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Xrad} & \Xrad & \texttt{\textbackslash NIL} & \NIL & \texttt{\textbackslash mip} & \mip \\
\texttt{\textbackslash neutroneq} & \neutroneq & \texttt{\textbackslash neqcmcm} & \neqcmcm & \texttt{\textbackslash kRad} & \kRad \\
\texttt{\textbackslash MRad} & \MRad & \texttt{\textbackslash ci} & \ci & \texttt{\textbackslash mci} & \mci \\
\end{tabular*}

\subsubsection{Uncertainties}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sx} & \sx & \texttt{\textbackslash sy} & \sy & \texttt{\textbackslash sz} & \sz \\
\texttt{\textbackslash stat} & \stat & \texttt{\textbackslash syst} & \syst &  \\
\end{tabular*}

\subsubsection{Maths}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash order} & \order & \texttt{\textbackslash chisq} & \chisq & \texttt{\textbackslash chisqndf} & \chisqndf \\
\texttt{\textbackslash chisqip} & \chisqip & \texttt{\textbackslash chisqvs} & \chisqvs & \texttt{\textbackslash chisqvtx} & \chisqvtx \\
\texttt{\textbackslash chisqvtxndf} & \chisqvtxndf & \texttt{\textbackslash deriv} & \deriv & \texttt{\textbackslash gsim} & \gsim \\
\texttt{\textbackslash lsim} & \lsim & \texttt{\textbackslash mean[1] \textbackslash mean\{x\}} & \mean{x} & \texttt{\textbackslash abs[1] \textbackslash abs\{x\}} & \abs{x} \\
\texttt{\textbackslash Real} & \Real & \texttt{\textbackslash Imag} & \Imag & \texttt{\textbackslash PDF} & \PDF \\
\texttt{\textbackslash sPlot} & \sPlot &  \\
\end{tabular*}

\subsection{Kinematics}
\subsubsection{Energy, Momenta}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Ebeam} & \Ebeam & \texttt{\textbackslash sqs} & \sqs & \texttt{\textbackslash ptot} & \ptot \\
\texttt{\textbackslash pt} & \pt & \texttt{\textbackslash et} & \et & \texttt{\textbackslash mt} & \mt \\
\texttt{\textbackslash dpp} & \dpp & \texttt{\textbackslash msq} & \msq & \texttt{\textbackslash dedx} & \dedx \\
\end{tabular*}

\subsubsection{PID}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dllkpi} & \dllkpi & \texttt{\textbackslash dllppi} & \dllppi & \texttt{\textbackslash dllepi} & \dllepi \\
\texttt{\textbackslash dllmupi} & \dllmupi &  \\
\end{tabular*}

\subsubsection{Geometry}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degrees} & \degrees & \texttt{\textbackslash krad} & \krad & \texttt{\textbackslash mrad} & \mrad \\
\texttt{\textbackslash rad} & \rad &  \\
\end{tabular*}

\subsubsection{Accelerator}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash betastar} & \betastar & \texttt{\textbackslash lum} & \lum & \texttt{\textbackslash intlum[1] \textbackslash intlum\{2 \,\invfb\}} & \intlum{2 \,\invfb} \\
\end{tabular*}

\subsection{Software}
\subsubsection{Programs}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bcvegpy} & \bcvegpy & \texttt{\textbackslash boole} & \boole & \texttt{\textbackslash brunel} & \brunel \\
\texttt{\textbackslash davinci} & \davinci & \texttt{\textbackslash dirac} & \dirac & \texttt{\textbackslash evtgen} & \evtgen \\
\texttt{\textbackslash fewz} & \fewz & \texttt{\textbackslash fluka} & \fluka & \texttt{\textbackslash ganga} & \ganga \\
\texttt{\textbackslash gaudi} & \gaudi & \texttt{\textbackslash gauss} & \gauss & \texttt{\textbackslash geant} & \geant \\
\texttt{\textbackslash hepmc} & \hepmc & \texttt{\textbackslash herwig} & \herwig & \texttt{\textbackslash moore} & \moore \\
\texttt{\textbackslash neurobayes} & \neurobayes & \texttt{\textbackslash photos} & \photos & \texttt{\textbackslash powheg} & \powheg \\
\texttt{\textbackslash pythia} & \pythia & \texttt{\textbackslash resbos} & \resbos & \texttt{\textbackslash roofit} & \roofit \\
\texttt{\textbackslash root} & \root & \texttt{\textbackslash spice} & \spice & \texttt{\textbackslash urania} & \urania \\
\end{tabular*}

\subsubsection{Languages}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cpp} & \cpp & \texttt{\textbackslash ruby} & \ruby & \texttt{\textbackslash fortran} & \fortran \\
\texttt{\textbackslash svn} & \svn &  \\
\end{tabular*}

\subsubsection{Data processing}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash kbytes} & \kbytes & \texttt{\textbackslash kbsps} & \kbsps & \texttt{\textbackslash kbits} & \kbits \\
\texttt{\textbackslash kbsps} & \kbsps & \texttt{\textbackslash mbsps} & \mbsps & \texttt{\textbackslash mbytes} & \mbytes \\
\texttt{\textbackslash mbps} & \mbps & \texttt{\textbackslash mbsps} & \mbsps & \texttt{\textbackslash gbsps} & \gbsps \\
\texttt{\textbackslash gbytes} & \gbytes & \texttt{\textbackslash gbsps} & \gbsps & \texttt{\textbackslash tbytes} & \tbytes \\
\texttt{\textbackslash tbpy} & \tbpy & \texttt{\textbackslash dst} & \dst &  \\
\end{tabular*}

\subsection{Detector related}
\subsubsection{Detector technologies}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash nonn} & \nonn & \texttt{\textbackslash ponn} & \ponn & \texttt{\textbackslash nonp} & \nonp \\
\texttt{\textbackslash cvd} & \cvd & \texttt{\textbackslash mwpc} & \mwpc & \texttt{\textbackslash gem} & \gem \\
\end{tabular*}

\subsubsection{Detector components, electronics}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tell1} & \tell1 & \texttt{\textbackslash ukl1} & \ukl1 & \texttt{\textbackslash beetle} & \beetle \\
\texttt{\textbackslash otis} & \otis & \texttt{\textbackslash croc} & \croc & \texttt{\textbackslash carioca} & \carioca \\
\texttt{\textbackslash dialog} & \dialog & \texttt{\textbackslash sync} & \sync & \texttt{\textbackslash cardiac} & \cardiac \\
\texttt{\textbackslash gol} & \gol & \texttt{\textbackslash vcsel} & \vcsel & \texttt{\textbackslash ttc} & \ttc \\
\texttt{\textbackslash ttcrx} & \ttcrx & \texttt{\textbackslash hpd} & \hpd & \texttt{\textbackslash pmt} & \pmt \\
\texttt{\textbackslash specs} & \specs & \texttt{\textbackslash elmb} & \elmb & \texttt{\textbackslash fpga} & \fpga \\
\texttt{\textbackslash plc} & \plc & \texttt{\textbackslash rasnik} & \rasnik & \texttt{\textbackslash elmb} & \elmb \\
\texttt{\textbackslash can} & \can & \texttt{\textbackslash lvds} & \lvds & \texttt{\textbackslash ntc} & \ntc \\
\texttt{\textbackslash adc} & \adc & \texttt{\textbackslash led} & \led & \texttt{\textbackslash ccd} & \ccd \\
\texttt{\textbackslash hv} & \hv & \texttt{\textbackslash lv} & \lv & \texttt{\textbackslash pvss} & \pvss \\
\texttt{\textbackslash cmos} & \cmos & \texttt{\textbackslash fifo} & \fifo & \texttt{\textbackslash ccpc} & \ccpc \\
\end{tabular*}

\subsubsection{Chemical symbols}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cfourften} & \cfourften & \texttt{\textbackslash cffour} & \cffour & \texttt{\textbackslash cotwo} & \cotwo \\
\texttt{\textbackslash csixffouteen} & \csixffouteen & \texttt{\textbackslash mgftwo} & \mgftwo & \texttt{\textbackslash siotwo} & \siotwo \\
\end{tabular*}

\subsection{Special Text }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eg} & \eg & \texttt{\textbackslash ie} & \ie & \texttt{\textbackslash etal} & \etal \\
\texttt{\textbackslash etc} & \etc & \texttt{\textbackslash cf} & \cf & \texttt{\textbackslash ffp} & \ffp \\
\texttt{\textbackslash vs} & \vs &  \\
\end{tabular*}



==> listsymbols <==
#!/bin/env python
import re

class TableWrite:
    """Write tables with correct header and footer"""
    
    def __init__(self,file):
        self.f = file
        self.columncount = 0
        self.tableopen= False
        self.tablebegin = r'\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}'+'\n'
        self.tableend=r'\end{tabular*}'+'\n'

    def item(self,text):
        if not self.tableopen:
            self.f.write(self.tablebegin)
            self.tableopen=True
            self.columncount = 0
        self.f.write(text)
        if self.columncount<2:
            self.f.write(' & ')
            self.columncount+=1
        else:
            self.f.write(r' \\'+'\n')
            self.columncount=0

    def finish(self):
        if self.tableopen:
            if self.columncount>0:
                self.f.write(r' \\'+'\n')
            self.f.write(self.tableend+'\n')
            self.tableopen=False

    def header(self,text):
        self.finish()
        self.f.write(text+'\n')

fin = open('lhcb-symbols-def.tex')
outname = 'lhcb-symbols-list.tex'
fout = open(outname,'w')
print "All symbols are now available in the file %s." % outname

fout.write("""% This is an automatically generated appendix to template.tex. 
% When included it will show all the symbols defined in lhcb-symbols-def.tex.
%
% To regenerate with the latest definitions run the script ./listsymbols

\\section{List of all symbols}
\\label{sec:listofsymbols}
""")

psection = re.compile(r'(%+)\s*(.*)')
pdef = re.compile(r'^\\def(\\.+?)[\s{]+[^%]*(%\s.+)*')
pnew = re.compile(r'^\\newcommand\{(\\\w+?)\}(\[\d\])*[\s\{]+[^%]*(%\s.+)*')
parg = re.compile(r'.+(#\d)+.*')

writer=TableWrite(fout)

for l in fin.readlines():

    # Match on section headers
    m = psection.match(l)
    if m:
        length = len(m.group(1))
        if length<=2:
            if length==1:
                writer.header('\\subsection{%s}' % m.group(2))
            else:
                writer.header('\\subsubsection{%s}' % m.group(2))

    # Match on the \def lines
    m = pdef.match(l)
    if m:
        marg = parg.match(m.group(1))
        if not marg:
            writer.item('\\texttt{\\textbackslash %s} & %s' 
                        % (m.group(1)[1:],m.group(1)))
        else:
            if m.group(2):
                pat1 = re.compile(r'#')
                pat2 = re.compile(r'(#\d)+')
                generic = re.sub(pat1,r'\#',m.group(1))
                example = re.sub(pat2,m.group(2)[2:],m.group(1))
                writer.item('\\texttt{\\textbackslash %s ' % generic[1:] +
                            '\\textbackslash %s} & %s' 
                            % (example[1:],example))
            else:
                print 'Ignoring line: %s' % l[:-1]

    # Match on the \newcommand lines
    m = pnew.match(l)
    if m:
        if not m.group(2):
            writer.item('\\texttt{\\textbackslash %s} & %s' 
                        % (m.group(1)[1:],m.group(1)))
        elif m.group(3):
            generic = str(m.group(3)[2:]).replace('{',r'\{').replace('}',r'\}')
            writer.item('\\texttt{\\textbackslash %s%s ' % 
                       (m.group(1)[1:],m.group(2)) +
                        '\\textbackslash %s%s} & %s%s' 
                        % (m.group(1)[1:],generic,
                           m.group(1),m.group(3)[2:]))
        else:
            print 'Ignoring line: %s' % l[:-1]
            
writer.finish()

fin.close()
fout.close()


==> mycommands_italic.tex <==
% Beate's commands
\def\DC{chapter}
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\xces{\langle \chi^2\rangle_{ces}}
\def\iso{iso4}
\def\fgam{$F_{\gamma}$}
\def\bi{\begin{itemize}}
\def\ei{\end{itemize}}
\def\bc{\begin{center}}
\def\ec{\end{center}}
\def\and{\/\mbox{and}}
%%

\newcommand{\squishlist}{
 \begin{list}{$\bullet$}
  { \setlength{\itemsep}{0pt}
     \setlength{\parsep}{3pt}
     \setlength{\topsep}{3pt}
     \setlength{\partopsep}{0pt}
     \setlength{\leftmargin}{1.5em}
     \setlength{\labelwidth}{1em}
     \setlength{\labelsep}{0.5em} } }

\newcommand{\squishlisttwo}{
 \begin{list}{$\bullet$}
  { \setlength{\itemsep}{0pt}
     \setlength{\parsep}{0pt}
    \setlength{\topsep}{0pt}
    \setlength{\partopsep}{0pt}
    \setlength{\leftmargin}{2em}
    \setlength{\labelwidth}{1.5em}
    \setlength{\labelsep}{0.5em} } }

\newcommand{\squishend}{
  \end{list}  }

\def\bvec#1{\vec{\bf #1}}
\newcommand{\uni}{Universit\a`a \,}
\newcommand{\rd}{{\rm d}}
\newcommand {\etjet} {E_t^{\rm jet}}
\newcommand {\etgam} {E_t^{\gamma}}
\newcommand {\etem} {E_t^{EM}}
\newcommand {\praw}  {P_{\rm raw}(\etjet)}
\newcommand {\prawem}  {P_{\rm raw}(\etem)}
\newcommand {\fgamma}  {F_\gamma}
\newcommand {\fqcd}  {F_{QCD}}

\newcommand {\ptruew} {P^W_{{\rm jet} \to \gamma}(\etjet)}
\newcommand {\ptruej} {P^j_{{\rm jet} \to \gamma}(\etjet)}
\newcommand {\ptrue} {P_{{\rm jet} \to \gamma}(\etjet)}
\newcommand {\ptrueem} {P_{{\rm EM} \to \gamma}(\etem)}

\newcommand {\njet}  {N_{\rm jet}}
%\newcommand{\met}{E\!\!\!/_t }
\newcommand{\mee}{M_{ee}}
\newcommand{\mll}{M_{\ell\ell}}
\newcommand{\gammacand}{\gamma - candidate}
\newcommand{\TeV}{\ensuremath{\mathrm{Te\kern -0.1em V}}}
\newcommand{\GeV}{\ensuremath{\mathrm{Ge\kern -0.1em V}}}
\newcommand{\MeV}{\ensuremath{\mathrm{Me\kern -0.1em V}}}
\newcommand{\Tesla}{\ensuremath{\mathrm{T}}}
%\newcommand{\cm}{\ensuremath{\mathrm{cm}}}
\newcommand{\um}{\ensuremath{\mathrm{\mu m}}}
\newcommand{\us}{\ensuremath{\mathrm{\mu s}}}
%\newcommand{\ps}{\ensuremath{\mathrm{ps}}}
\newcommand{\at}{\symbol{64}}
\newcommand{\sye}[1]{\ensuremath{~\pm #1}}
\newcommand{\ase}[2]{\ensuremath{^{~+ #1}_{~- #2}}}
\newcommand{\asi}[2]{\ensuremath{^{~- #1}_{~+ #2}}}
\newcommand{\MeVCSq}{\ensuremath{\MeV\!/c^2}}
\newcommand{\GeVCSq}{\ensuremath{\GeV\!/c^2}}
\newcommand{\TeVCSq}{\ensuremath{\TeV\!/c^2}}
\newcommand{\GeVC}{\ensuremath{\GeV\!/c}}
\newcommand{\zg}{{ Z}^0/\gamma^*}
\newcommand{\zll}{{ Z}^0\rightarrow{ \ell}^+ { \ell}^-}
\newcommand{\zgll}{{ Z}^0/\gamma^*\rightarrow{ \ell}^+ { \ell}^-}
\newcommand{\wlnu}{{ W^{\pm}} \rightarrow{ \ell}^{\pm}\nu} 
\newcommand{\zgee}{{ Z}^0/\gamma^*\rightarrow{ e}^+ { e}^-}
\newcommand{\zee}{{ Z}^0\rightarrow{ e}^+ { e}^-}
\newcommand{\zmm}{{ Z}^0\rightarrow{ \mu}^+ { \mu}^-}
\newcommand{\ztt}{{ Z}^0\rightarrow{ \tau}^+ { \tau}^-}
\newcommand{\zgtt}{{ Z}^0/\gamma^*\rightarrow{ \tau}^+ { \tau}^-}
\newcommand{\zgmm}{{ Z}^0/\gamma^*\rightarrow{ \mu}^+ { \mu}^-}
\newcommand{\zttee}{{ Z}^0/\gamma^*\rightarrow\tau^+\tau^-\rightarrow { e^+}\nu_e{\bar \nu_\tau} { e^-} \bar{\nu_e}\nu_\tau}
%\newcommand{\t}{t}
\newcommand{\boldit}{\bf}
\newcommand{\Qbar}{\bar{Q}}
%\newcommand{\t}{t}
\newcommand{\tbar}{\bar{t}}
\newcommand{\Wmp}{ W^{\mp}}
%\newcommand{\Wpm}{ W^{\pm}}
\newcommand{\wenu}{{ W^{\pm}} \rightarrow{ e}^{\pm}\nu} 
\newcommand{\wmnu}{{ W^{\pm}} \rightarrow{ \mu}^{\pm}\nu} 
\newcommand{\wtnu}{{ W^{\pm}} \rightarrow{ \tau}^{\pm}\nu} 
\newcommand{\ratioe}{\sigma({ p} \bar{ p} \rightarrow { W}^\pm
\rightarrow { e}^\pm \nu) / \sigma({ p} \bar{ p} \rightarrow {
Z^0} \rightarrow { e}^+ { e}^-)}
\newcommand{\ratiom}{\sigma({ p} \bar{ p} \rightarrow { W}^\pm
\rightarrow { \mu}^\pm \nu) / \sigma({ p} \bar{ p} \rightarrow {
Z^0} \rightarrow { \mu}^+ { \mu}^-)}
\newcommand{\sigmawen}{\sigma_{ W^\pm}}
\newcommand{\sigmazee}{\sigma_{ Z^0}}
\newcommand{\sigmabrwen}{\sigma_{ W^\pm}\cdot Br(\wenu)}
\newcommand{\sigmabrzee}{\sigma_{ Z^0}\cdot Br(\zee)}
\newcommand{\gam}{\Gamma({ W})}
\newcommand{\gamenu}{\Gamma({ W^\pm}\rightarrow { e^\pm}\nu)}
\newcommand{\gammnu}{\Gamma({ W^\pm}\rightarrow { \mu^\pm}\nu)}
%\newcommand{\met}{\not \! \! E_{ \rm T}}
%\newcommand{\et}{\ensuremath{E_{\rm T}}}
%\newcommand{\pt}{\ensuremath{p_{\rm T}}}

\newcommand{\ppbar} {p\overline{p}}
\newcommand{\pbinv} {{\mathrm{pb}^{-1}}}
\newcommand{\fbinv} {{\mathrm{fb}^{-1}}}
%\newcommand{\lum} {{\cal L}}

\newcommand {\gt}     {\mbox{$>$}}
\newcommand {\gea}    {\mbox{$>=$}}
\newcommand {\lea}    {\mbox{$<=$}}
\newcommand {\lt}     {\mbox{$<$}}
\newcommand {\rarr}     {\mbox{$~\rightarrow~$}}
\newcommand {\metp}   {\mbox{${\rm \not\! E}_{\rm T}$}}
\newcommand {\abseta} {\mbox{$\mid \eta \mid $}}

\newcommand{\bsmm}{$B^{0}_{s}\rightarrow \mu^+\mu^-\:$ }
\newcommand{\jpsi}{J/\psi}
\newcommand{\Wenu}{$W\rightarrow e\nu\:$ }
\newcommand{\Wtaunu}{$W\rightarrow \tau\nu\:$ }
\newcommand{\Wnjet}{W $+$ n jets$\:$}
\newcommand{\Wnojet}{W $+ 0$ jets$\:$}
\newcommand{\Zee}{{\it Z}$^0\rightarrow e^{+} e^{-}\:$ }
\newcommand{\Zgee}{{\it Z}$^0/\gamma^*\rightarrow e^{+} e^{-}\:$ }
\newcommand{\met}{\mbox{${\hbox{$E$\kern-0.6em\lower-.1ex\hbox{/}}}_{\rm T}\:$}}
\newcommand{\metx}{\mbox{${\hbox{$E$\kern-0.6em\lower-.1ex\hbox{/}}}_T\:$}}
\newcommand{\mety}{\mbox{${\hbox{$E$\kern-0.6em\lower-.1ex\hbox{/}}}_T\:$}}
\newcommand{\Zuu}{{\it Z}$\rightarrow \mu^{+} \mu^{-}\:$ }
\newcommand{\Wunu}{$W\rightarrow \mu \nu\:$ }

\newcommand{\etal} {{\em et al.}}
\newcommand{\ie} {{\em i.e.}}
\newcommand{\notedate}[1] {(#1)}

\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}
\newcommand{\bce}{\begin{center}}
\newcommand{\beqn}{\begin{eqnarray*}}
\newcommand{\eeqn}{\end{eqnarray*}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\ece}{\end{center}}
\newcommand{\rg}{\rightarrow} 

\newcommand{\mo}{$m_{0}\,$}
\newcommand{\azero}{$A_{0}\,$}
\newcommand{\miz}{$m_{1/2}\,$}
\newcommand{\tb}{$tan\beta\,$}
\newcommand{\ntwo}{\tilde{{\chi}}^{0}_{2}}
\newcommand{\cone}{\tilde{{\chi}}^\pm_{1}}
\newcommand{\none}{\tilde{{\chi}}^{0}_{1}}
\newcommand{\is}{{\scshape{Isajet }}}
\newcommand{\iss}{{\scshape{Isasusy }}}
\newcommand{\isg}{{\scshape{Isasugra }}}
\newcommand{\py}{{\scshape{Pythia }}}
\newcommand{\pro}{{\scshape{Prospino }}}
\newcommand{\ges}{\raisebox{-.7ex}{$\stackrel{\textstyle >}{\sim}$}}
\newcommand{\les}{\raisebox{-.7ex}{$\stackrel{\textstyle <}{\sim}$}}



==> mycommands_italic_lhcb.tex <==
% Beate's commands
\def\DC{chapter}
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\xces{\langle \chi^2\rangle_{ces}}
\def\iso{iso4}
\def\fgam{$F_{\gamma}$}
\def\bi{\begin{itemize}}
\def\ei{\end{itemize}}
\def\bc{\begin{center}}
\def\ec{\end{center}}
\def\and{\/\mbox{and}}
%%

\newcommand{\squishlist}{
 \begin{list}{$\bullet$}
  { \setlength{\itemsep}{0pt}
     \setlength{\parsep}{3pt}
     \setlength{\topsep}{3pt}
     \setlength{\partopsep}{0pt}
     \setlength{\leftmargin}{1.5em}
     \setlength{\labelwidth}{1em}
     \setlength{\labelsep}{0.5em} } }

\newcommand{\squishlisttwo}{
 \begin{list}{$\bullet$}
  { \setlength{\itemsep}{0pt}
     \setlength{\parsep}{0pt}
    \setlength{\topsep}{0pt}
    \setlength{\partopsep}{0pt}
    \setlength{\leftmargin}{2em}
    \setlength{\labelwidth}{1.5em}
    \setlength{\labelsep}{0.5em} } }

\newcommand{\squishend}{
  \end{list}  }

\def\bvec#1{\vec{\bf #1}}
\newcommand{\uni}{Universit\a`a \,}
\newcommand{\rd}{{\rm d}}
\newcommand {\etjet} {E_t^{\rm jet}}
\newcommand {\etgam} {E_t^{\gamma}}
\newcommand {\etem} {E_t^{EM}}
\newcommand {\praw}  {P_{\rm raw}(\etjet)}
\newcommand {\prawem}  {P_{\rm raw}(\etem)}
\newcommand {\fgamma}  {F_\gamma}
\newcommand {\fqcd}  {F_{QCD}}

\newcommand {\ptruew} {P^W_{{\rm jet} \to \gamma}(\etjet)}
\newcommand {\ptruej} {P^j_{{\rm jet} \to \gamma}(\etjet)}
\newcommand {\ptrue} {P_{{\rm jet} \to \gamma}(\etjet)}
\newcommand {\ptrueem} {P_{{\rm EM} \to \gamma}(\etem)}

\newcommand {\njet}  {N_{\rm jet}}
%\newcommand{\met}{E\!\!\!/_t }
\newcommand{\mee}{M_{ee}}
\newcommand{\mll}{M_{\ell\ell}}
\newcommand{\gammacand}{\gamma - candidate}
\newcommand{\TeV}{\ensuremath{\mathrm{Te\kern -0.1em V}}}
\newcommand{\GeV}{\ensuremath{\mathrm{Ge\kern -0.1em V}}}
\newcommand{\MeV}{\ensuremath{\mathrm{Me\kern -0.1em V}}}
\newcommand{\Tesla}{\ensuremath{\mathrm{T}}}
%\newcommand{\cm}{\ensuremath{\mathrm{cm}}}
\newcommand{\um}{\ensuremath{\mathrm{\mu m}}}
\newcommand{\us}{\ensuremath{\mathrm{\mu s}}}
%\newcommand{\ps}{\ensuremath{\mathrm{ps}}}
\newcommand{\at}{\symbol{64}}
\newcommand{\sye}[1]{\ensuremath{~\pm #1}}
\newcommand{\ase}[2]{\ensuremath{^{~+ #1}_{~- #2}}}
\newcommand{\asi}[2]{\ensuremath{^{~- #1}_{~+ #2}}}
\newcommand{\MeVCSq}{\ensuremath{\MeV\!/c^2}}
\newcommand{\GeVCSq}{\ensuremath{\GeV\!/c^2}}
\newcommand{\TeVCSq}{\ensuremath{\TeV\!/c^2}}
\newcommand{\GeVC}{\ensuremath{\GeV\!/c}}
\newcommand{\zg}{{ Z}^0/\gamma^*}
\newcommand{\zll}{{ Z}^0\rightarrow{ \ell}^+ { \ell}^-}
\newcommand{\zgll}{{ Z}^0/\gamma^*\rightarrow{ \ell}^+ { \ell}^-}
\newcommand{\wlnu}{{ W^{\pm}} \rightarrow{ \ell}^{\pm}\nu} 
\newcommand{\zgee}{{ Z}^0/\gamma^*\rightarrow{ e}^+ { e}^-}
\newcommand{\zee}{{ Z}^0\rightarrow{ e}^+ { e}^-}
\newcommand{\zmm}{{ Z}^0\rightarrow{ \mu}^+ { \mu}^-}
\newcommand{\ztt}{{ Z}^0\rightarrow{ \tau}^+ { \tau}^-}
\newcommand{\zgtt}{{ Z}^0/\gamma^*\rightarrow{ \tau}^+ { \tau}^-}
\newcommand{\zgmm}{{ Z}^0/\gamma^*\rightarrow{ \mu}^+ { \mu}^-}
\newcommand{\zttee}{{ Z}^0/\gamma^*\rightarrow\tau^+\tau^-\rightarrow { e^+}\nu_e{\bar \nu_\tau} { e^-} \bar{\nu_e}\nu_\tau}
%\newcommand{\t}{t}
\newcommand{\boldit}{\bf}
\newcommand{\Qbar}{\bar{Q}}
%\newcommand{\t}{t}
\newcommand{\tbar}{\bar{t}}
\newcommand{\Wmp}{ W^{\mp}}
%\newcommand{\Wpm}{ W^{\pm}}
\newcommand{\wenu}{{ W^{\pm}} \rightarrow{ e}^{\pm}\nu} 
\newcommand{\wmnu}{{ W^{\pm}} \rightarrow{ \mu}^{\pm}\nu} 
\newcommand{\wtnu}{{ W^{\pm}} \rightarrow{ \tau}^{\pm}\nu} 
\newcommand{\ratioe}{\sigma({ p} \bar{ p} \rightarrow { W}^\pm
\rightarrow { e}^\pm \nu) / \sigma({ p} \bar{ p} \rightarrow {
Z^0} \rightarrow { e}^+ { e}^-)}
\newcommand{\ratiom}{\sigma({ p} \bar{ p} \rightarrow { W}^\pm
\rightarrow { \mu}^\pm \nu) / \sigma({ p} \bar{ p} \rightarrow {
Z^0} \rightarrow { \mu}^+ { \mu}^-)}
\newcommand{\sigmawen}{\sigma_{ W^\pm}}
\newcommand{\sigmazee}{\sigma_{ Z^0}}
\newcommand{\sigmabrwen}{\sigma_{ W^\pm}\cdot Br(\wenu)}
\newcommand{\sigmabrzee}{\sigma_{ Z^0}\cdot Br(\zee)}
\newcommand{\gam}{\Gamma({ W})}
\newcommand{\gamenu}{\Gamma({ W^\pm}\rightarrow { e^\pm}\nu)}
\newcommand{\gammnu}{\Gamma({ W^\pm}\rightarrow { \mu^\pm}\nu)}
%\newcommand{\met}{\not \! \! E_{ \rm T}}
%\newcommand{\et}{\ensuremath{E_{\rm T}}}
%\newcommand{\pt}{\ensuremath{p_{\rm T}}}

\newcommand{\ppbar} {p\overline{p}}
\newcommand{\pbinv} {{\mathrm{pb}^{-1}}}
\newcommand{\fbinv} {{\mathrm{fb}^{-1}}}
%\newcommand{\lum} {{\cal L}}

\newcommand {\gt}     {\mbox{$>$}}
\newcommand {\gea}    {\mbox{$>=$}}
\newcommand {\lea}    {\mbox{$<=$}}
\newcommand {\lt}     {\mbox{$<$}}
\newcommand {\rarr}     {\mbox{$~\rightarrow~$}}
\newcommand {\metp}   {\mbox{${\rm \not\! E}_{\rm T}$}}
\newcommand {\abseta} {\mbox{$\mid \eta \mid $}}

\newcommand{\bsmm}{$B^{0}_{s}\rightarrow \mu^+\mu^-\:$ }
%\newcommand{\jpsi}{J/\psi}
\newcommand{\Wenu}{$W\rightarrow e\nu\:$ }
\newcommand{\Wtaunu}{$W\rightarrow \tau\nu\:$ }
\newcommand{\Wnjet}{W $+$ n jets$\:$}
\newcommand{\Wnojet}{W $+ 0$ jets$\:$}
\newcommand{\Zee}{{\it Z}$^0\rightarrow e^{+} e^{-}\:$ }
\newcommand{\Zgee}{{\it Z}$^0/\gamma^*\rightarrow e^{+} e^{-}\:$ }
\newcommand{\met}{\mbox{${\hbox{$E$\kern-0.6em\lower-.1ex\hbox{/}}}_{\rm T}\:$}}
\newcommand{\metx}{\mbox{${\hbox{$E$\kern-0.6em\lower-.1ex\hbox{/}}}_T\:$}}
\newcommand{\mety}{\mbox{${\hbox{$E$\kern-0.6em\lower-.1ex\hbox{/}}}_T\:$}}
\newcommand{\Zuu}{{\it Z}$\rightarrow \mu^{+} \mu^{-}\:$ }
\newcommand{\Wunu}{$W\rightarrow \mu \nu\:$ }

%\newcommand{\etal} {{\em et al.}}
%\newcommand{\ie} {{\em i.e.}}
\newcommand{\notedate}[1] {(#1)}

\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}
\newcommand{\bce}{\begin{center}}
\newcommand{\beqn}{\begin{eqnarray*}}
\newcommand{\eeqn}{\end{eqnarray*}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\ece}{\end{center}}
\newcommand{\rg}{\rightarrow} 

\newcommand{\mo}{$m_{0}\,$}
\newcommand{\azero}{$A_{0}\,$}
\newcommand{\miz}{$m_{1/2}\,$}
\newcommand{\tb}{$tan\beta\,$}
\newcommand{\ntwo}{\tilde{{\chi}}^{0}_{2}}
\newcommand{\cone}{\tilde{{\chi}}^\pm_{1}}
\newcommand{\none}{\tilde{{\chi}}^{0}_{1}}
\newcommand{\is}{{\scshape{Isajet }}}
\newcommand{\iss}{{\scshape{Isasusy }}}
\newcommand{\isg}{{\scshape{Isasugra }}}
\newcommand{\py}{{\scshape{Pythia }}}
\newcommand{\pro}{{\scshape{Prospino }}}
\newcommand{\ges}{\raisebox{-.7ex}{$\stackrel{\textstyle >}{\sim}$}}
\newcommand{\les}{\raisebox{-.7ex}{$\stackrel{\textstyle <}{\sim}$}}



==> tables/CrossSection2D.tex <==
Forward&&&&&\\
$\pt[\gevc]$ &$1.5<y^*<2.0$   &$2.0<y^*<2.5$    &$2.5<y^*<3.0$     &$3.0<y^*<3.5$     &$3.5<y^*<4.0$\\
\hline
$[0,1]$&$6.835\pm1.131\pm0.590\pm0.528$	&$7.069\pm0.207\pm0.104\pm0.766$	&$7.953\pm0.164\pm0.085\pm0.659$	&$7.527\pm0.185\pm0.091\pm0.393$	&$7.132\pm0.270\pm0.134\pm0.468$	\\
$[1,2]$&$11.748\pm0.481\pm0.282\pm0.848$	&$12.768\pm0.157\pm0.092\pm1.079$	&$12.198\pm0.122\pm0.069\pm0.806$	&$10.733\pm0.130\pm0.071\pm0.609$	&$8.238\pm0.187\pm0.091\pm0.487$	\\
$[2,3]$&$8.377\pm0.165\pm0.102\pm0.527$	&$8.348\pm0.067\pm0.041\pm0.671$	&$7.552\pm0.054\pm0.032\pm0.704$	&$6.096\pm0.054\pm0.034\pm0.523$	&$4.476\pm0.075\pm0.039\pm0.307$	\\
$[3,4]$&$4.383\pm0.069\pm0.044\pm0.274$	&$4.067\pm0.032\pm0.018\pm0.500$	&$3.678\pm0.027\pm0.016\pm0.539$	&$2.873\pm0.027\pm0.015\pm0.379$	&$2.040\pm0.037\pm0.019\pm0.178$	\\
$[4,5]$&$2.103\pm0.034\pm0.020\pm0.156$	&$2.015\pm0.018\pm0.010\pm0.338$	&$1.704\pm0.016\pm0.009\pm0.321$	&$1.238\pm0.015\pm0.008\pm0.216$	&$0.805\pm0.021\pm0.009\pm0.081$	\\
$[5,6]$&$1.108\pm0.020\pm0.012\pm0.099$	&$0.999\pm0.012\pm0.006\pm0.204$	&$0.808\pm0.010\pm0.005\pm0.183$	&$0.601\pm0.010\pm0.005\pm0.124$	&$0.348\pm0.015\pm0.006\pm0.033$	\\
$[6,7]$&$0.550\pm0.012\pm0.007\pm0.059$	&$0.494\pm0.008\pm0.004\pm0.115$	&$0.412\pm0.007\pm0.003\pm0.103$	&$0.294\pm0.007\pm0.003\pm0.064$	&$0.170\pm0.013\pm0.005\pm0.017$	\\
$[7,8]$&$0.318\pm0.009\pm0.005\pm0.038$	&$0.267\pm0.005\pm0.003\pm0.067$	&$0.231\pm0.005\pm0.002\pm0.061$	&$0.144\pm0.005\pm0.002\pm0.030$	&$0.073\pm0.015\pm0.005\pm0.009$	\\
$[8,9]$&$0.188\pm0.006\pm0.004\pm0.025$	&$0.154\pm0.004\pm0.002\pm0.041$	&$0.133\pm0.004\pm0.002\pm0.037$	&$0.084\pm0.004\pm0.002\pm0.016$	&$-$	\\
$[9,10]$&$0.111\pm0.005\pm0.002\pm0.017$	&$0.094\pm0.003\pm0.001\pm0.026$	&$0.072\pm0.003\pm0.001\pm0.021$	&$0.052\pm0.004\pm0.002\pm0.008$	&$-$	\\
$[10,11]$&$0.066\pm0.003\pm0.002\pm0.011$	&$0.056\pm0.002\pm0.001\pm0.016$	&$0.043\pm0.002\pm0.001\pm0.012$	&$0.028\pm0.004\pm0.002\pm0.004$	&$-$	\\
$[11,12]$&$0.043\pm0.003\pm0.001\pm0.007$	&$0.040\pm0.002\pm0.001\pm0.011$	&$0.027\pm0.002\pm0.001\pm0.007$	&$0.026\pm0.004\pm0.003\pm0.005$	&$-$	\\
$[12,13]$&$0.022\pm0.002\pm0.001\pm0.004$	&$0.022\pm0.002\pm0.001\pm0.007$	&$0.019\pm0.002\pm0.001\pm0.005$	&$-$	&$-$	\\
$[13,14]$&$0.023\pm0.002\pm0.001\pm0.004$	&$0.014\pm0.001\pm0.001\pm0.004$	&$0.012\pm0.001\pm0.001\pm0.003$	&$-$	&$-$	\\
\hline
Backward&&&&&\\
$\pt[\gevc]$ &$-3.0<y^*<-2.5$   &$-3.5<y^*<-3.0$    &$-4.0<y^*<-3.5$     &$-4.5<y^*<-4.0$     &$-5.0<y^*<-4.5$\\
\hline
$[0,1]$&$6.430\pm1.127\pm0.371\pm0.647$	&$7.921\pm0.340\pm0.115\pm0.835$	&$9.220\pm0.321\pm0.106\pm0.607$	&$8.069\pm0.438\pm0.115\pm0.571$	&$8.054\pm0.750\pm0.195\pm0.715$	\\
$[1,2]$&$13.372\pm0.641\pm0.321\pm0.966$	&$13.751\pm0.252\pm0.099\pm1.162$	&$12.931\pm0.221\pm0.073\pm0.855$	&$11.049\pm0.283\pm0.073\pm0.627$	&$7.973\pm0.497\pm0.088\pm0.471$	\\
$[2,3]$&$8.325\pm0.210\pm0.101\pm0.524$	&$8.064\pm0.102\pm0.040\pm0.649$	&$7.087\pm0.087\pm0.030\pm0.661$	&$5.434\pm0.092\pm0.030\pm0.467$	&$3.603\pm0.138\pm0.032\pm0.247$	\\
$[3,4]$&$4.058\pm0.086\pm0.040\pm0.254$	&$3.616\pm0.046\pm0.016\pm0.445$	&$2.965\pm0.039\pm0.013\pm0.435$	&$2.017\pm0.038\pm0.011\pm0.266$	&$1.081\pm0.052\pm0.010\pm0.094$	\\
$[4,5]$&$1.824\pm0.042\pm0.018\pm0.135$	&$1.533\pm0.024\pm0.008\pm0.257$	&$1.194\pm0.021\pm0.006\pm0.225$	&$0.775\pm0.020\pm0.005\pm0.135$	&$0.338\pm0.026\pm0.004\pm0.034$	\\
$[5,6]$&$0.857\pm0.024\pm0.009\pm0.077$	&$0.702\pm0.015\pm0.004\pm0.144$	&$0.492\pm0.012\pm0.003\pm0.111$	&$0.294\pm0.011\pm0.002\pm0.060$	&$0.094\pm0.017\pm0.002\pm0.009$	\\
$[6,7]$&$0.433\pm0.015\pm0.006\pm0.046$	&$0.340\pm0.009\pm0.003\pm0.079$	&$0.227\pm0.008\pm0.002\pm0.057$	&$0.128\pm0.008\pm0.001\pm0.028$	&$-$	\\
$[7,8]$&$0.223\pm0.009\pm0.003\pm0.026$	&$0.159\pm0.006\pm0.002\pm0.040$	&$0.106\pm0.005\pm0.001\pm0.028$	&$0.053\pm0.005\pm0.001\pm0.011$	&$-$	\\
$[8,9]$&$0.120\pm0.007\pm0.002\pm0.016$	&$0.087\pm0.004\pm0.001\pm0.023$	&$0.055\pm0.004\pm0.001\pm0.015$	&$0.024\pm0.004\pm0.001\pm0.005$	&$-$	\\
$[9,10]$&$0.065\pm0.005\pm0.001\pm0.010$	&$0.051\pm0.003\pm0.001\pm0.014$	&$0.030\pm0.003\pm0.001\pm0.009$	&$0.014\pm0.004\pm0.001\pm0.002$	&$-$	\\
$[10,11]$&$0.042\pm0.004\pm0.001\pm0.007$	&$0.030\pm0.003\pm0.001\pm0.009$	&$0.014\pm0.002\pm0.000\pm0.004$	&$-$	&$-$	\\
$[11,12]$&$0.029\pm0.003\pm0.001\pm0.005$	&$0.014\pm0.002\pm0.000\pm0.004$	&$0.008\pm0.001\pm0.000\pm0.002$	&$-$	&$-$	\\
$[12,13]$&$0.021\pm0.002\pm0.001\pm0.004$	&$0.008\pm0.001\pm0.000\pm0.002$	&$-$	&$-$	&$-$	\\
$[13,14]$&$0.013\pm0.002\pm0.001\pm0.002$	&$0.006\pm0.001\pm0.000\pm0.002$	&$-$	&$-$	&$-$	\\


==> tables/p_CrossSection1DPT.tex <==
Forward [\mbarn/(\gevc)]&&&&&\\
$\pt[\gevc]$&$1.5<y^*<4.0$ &$2.5<y^*<4.0$ &$3.0<y^*<4.0$ &$2.5<y^*<3.5$ &$2.5<y^*<3.0$\\
\hline
$[0,1]$&$18.804\pm0.601\pm1.195$&$11.384\pm0.148\pm0.691$&$7.348\pm0.148\pm0.314$&$-$	&$-$	\\
$[1,2]$&$28.805\pm0.281\pm1.673$&$16.133\pm0.117\pm0.965$&$-$	&$-$	&$-$	\\
$[2,3]$&$18.116\pm0.104\pm1.012$&$9.488\pm0.052\pm0.532$&$-$	&$-$	&$-$	\\
$[3,4]$&$8.863\pm0.047\pm0.499$&$4.478\pm0.026\pm0.252$&$-$	&$-$	&$-$	\\
$[4,5]$&$4.114\pm0.025\pm0.232$&$2.007\pm0.015\pm0.113$&$-$	&$-$	&$-$	\\
$[5,6]$&$2.026\pm0.015\pm0.113$&$0.945\pm0.010\pm0.054$&$-$	&$-$	&$-$	\\
$[6,7]$&$1.015\pm0.011\pm0.059$&$0.472\pm0.008\pm0.027$&$-$	&$-$	&$-$	\\
$[7,8]$&$0.549\pm0.009\pm0.032$&$0.245\pm0.008\pm0.015$&$-$	&$-$	&$-$	\\
$[8,9]$&$0.293\pm0.005\pm0.017$&$0.116\pm0.003\pm0.007$&$-$	&$0.116\pm0.003\pm0.004$&$-$	\\
$[9,10]$&$0.171\pm0.004\pm0.010$&$0.064\pm0.002\pm0.004$&$-$	&$0.064\pm0.002\pm0.002$&$-$	\\
$[10,11]$&$0.101\pm0.003\pm0.006$&$0.037\pm0.002\pm0.002$&$-$	&$0.037\pm0.002\pm0.001$&$-$	\\
$[11,12]$&$0.071\pm0.003\pm0.005$&$0.028\pm0.003\pm0.002$&$-$	&$0.028\pm0.003\pm0.002$&$-$	\\
$[12,13]$&$0.033\pm0.001\pm0.002$&$0.010\pm0.001\pm0.001$&$-$	&$-$	&$0.010\pm0.001\pm0.001$\\
$[13,14]$&$0.027\pm0.001\pm0.002$&$0.006\pm0.001\pm0.001$&$-$	&$-$	&$0.006\pm0.001\pm0.000$\\
\hline
Backward [\mbarn/(\gevc)]&&&&&\\
$\pt[\gevc]$&$-5.0<y^*<-2.5$ &$-4.0<y^*<-2.5$ &$-4.0<y^*<-3.0$ &$-3.5<y^*<-2.5$ &$-3.0<y^*<-2.5$\\
\hline
$[0,1]$&$17.188\pm0.284\pm1.239$&$8.965\pm0.126\pm0.631$&$8.965\pm0.126\pm0.470$&$-$	&$-$	\\
$[1,2]$&$31.527\pm0.443\pm2.038$&$21.581\pm0.401\pm1.406$&$-$	&$-$	&$-$	\\
$[2,3]$&$17.651\pm0.148\pm1.088$&$12.714\pm0.128\pm0.772$&$-$	&$-$	&$-$	\\
$[3,4]$&$7.361\pm0.063\pm0.437$&$5.697\pm0.055\pm0.335$&$-$	&$-$	&$-$	\\
$[4,5]$&$3.056\pm0.031\pm0.181$&$2.446\pm0.027\pm0.143$&$-$	&$-$	&$-$	\\
$[5,6]$&$1.323\pm0.018\pm0.077$&$1.109\pm0.016\pm0.064$&$-$	&$-$	&$-$	\\
$[6,7]$&$0.604\pm0.011\pm0.036$&$0.534\pm0.010\pm0.032$&$-$	&$-$	&$-$	\\
$[7,8]$&$0.290\pm0.007\pm0.016$&$0.261\pm0.006\pm0.015$&$-$	&$-$	&$-$	\\
$[8,9]$&$0.156\pm0.005\pm0.010$&$0.143\pm0.005\pm0.008$&$-$	&$0.111\pm0.005\pm0.004$&$-$	\\
$[9,10]$&$0.078\pm0.003\pm0.005$&$0.078\pm0.003\pm0.005$&$-$	&$0.062\pm0.003\pm0.002$&$-$	\\
$[10,11]$&$0.048\pm0.003\pm0.003$&$0.048\pm0.003\pm0.003$&$-$	&$0.040\pm0.003\pm0.002$&$-$	\\
$[11,12]$&$0.027\pm0.002\pm0.002$&$0.027\pm0.002\pm0.002$&$-$	&$0.023\pm0.002\pm0.001$&$-$	\\
$[12,13]$&$0.015\pm0.001\pm0.001$&$0.015\pm0.001\pm0.001$&$-$	&$-$	&$0.011\pm0.001\pm0.001$\\
$[13,14]$&$0.010\pm0.001\pm0.001$&$0.010\pm0.001\pm0.001$&$-$	&$-$	&$0.007\pm0.001\pm0.000$\\


==> tables/p_CrossSection1DY.tex <==
Fwd\\
$y*$&$\pt[\gevc]$&$\frac{\deriv \sigma}{\deriv y^*}$ [\mbarn]\\
\hline
$[1.5,2.0]$&$[1,14]$&$30.00\pm0.52\pm0.32\pm1.72$\\
$[2.0,2.5]$&$[1,14]$&$30.31\pm0.17\pm0.11\pm1.67$\\
$[2.5,3.0]$&$[1,14]$&$27.66\pm0.13\pm0.10\pm1.52$\\
$[3.0,3.5]$&$[1,12]$&$23.38\pm0.13\pm0.10\pm1.32$\\
$[3.5,4.0]$&$[1,8]$&$17.02\pm0.19\pm0.16\pm1.01$\\
\hline
Bwd\\
$y*$&$\pt[\gevc]$&$\frac{\deriv \sigma}{\deriv y^*}$ [\mbarn]\\
\hline
$[-3.0,-2.5]$&$[1,14]$&$31.83\pm0.78\pm0.31\pm1.67$\\
$[-3.5,-3.0]$&$[1,14]$&$30.76\pm0.27\pm0.12\pm1.45$\\
$[-4.0,-3.5]$&$[1,12]$&$26.74\pm0.21\pm0.10\pm1.73$\\
$[-4.5,-4.0]$&$[1,9]$&$21.24\pm0.23\pm0.11\pm1.54$\\
$[-5.0,-4.5]$&$[1,6]$&$13.73\pm0.35\pm0.17\pm1.28$\\


==> tablesDs/CrossSection2D.tex <==
Forward&&&&&\\
$\pt[\gevc]$ &$1.5<y^*<2.0$   &$2.0<y^*<2.5$    &$2.5<y^*<3.0$     &$3.0<y^*<3.5$     &$3.5<y^*<4.0$\\
\hline
$[0,1]$&$-$	&$3.213\pm0.403\pm0.123\pm0.441$	&$2.873\pm0.346\pm0.097\pm0.317$	&$3.454\pm0.538\pm0.147\pm0.303$	&$2.134\pm1.045\pm0.175\pm0.205$	\\
$[1,2]$&$4.885\pm0.521\pm0.170\pm0.621$	&$5.250\pm0.227\pm0.073\pm0.602$	&$6.079\pm0.219\pm0.077\pm0.505$	&$4.464\pm0.235\pm0.072\pm0.356$	&$3.699\pm0.415\pm0.110\pm0.316$	\\
$[2,3]$&$4.059\pm0.221\pm0.078\pm0.487$	&$3.738\pm0.104\pm0.034\pm0.356$	&$3.640\pm0.094\pm0.034\pm0.318$	&$2.659\pm0.098\pm0.033\pm0.217$	&$1.630\pm0.149\pm0.038\pm0.133$	\\
$[3,4]$&$2.090\pm0.093\pm0.031\pm0.211$	&$1.967\pm0.052\pm0.018\pm0.218$	&$1.717\pm0.046\pm0.017\pm0.199$	&$1.248\pm0.046\pm0.016\pm0.130$	&$0.623\pm0.065\pm0.016\pm0.054$	\\
$[4,5]$&$1.096\pm0.051\pm0.017\pm0.101$	&$0.964\pm0.030\pm0.010\pm0.133$	&$0.817\pm0.027\pm0.009\pm0.118$	&$0.534\pm0.026\pm0.008\pm0.069$	&$0.315\pm0.035\pm0.008\pm0.029$	\\
$[5,6]$&$0.592\pm0.032\pm0.011\pm0.058$	&$0.509\pm0.020\pm0.006\pm0.081$	&$0.363\pm0.017\pm0.006\pm0.059$	&$0.226\pm0.016\pm0.004\pm0.034$	&$0.166\pm0.029\pm0.006\pm0.016$	\\
$[6,7]$&$0.275\pm0.019\pm0.007\pm0.029$	&$0.227\pm0.012\pm0.004\pm0.040$	&$0.196\pm0.012\pm0.004\pm0.035$	&$0.124\pm0.011\pm0.003\pm0.020$	&$0.090\pm0.022\pm0.005\pm0.009$	\\
$[7,8]$&$0.154\pm0.013\pm0.004\pm0.018$	&$0.108\pm0.008\pm0.002\pm0.020$	&$0.099\pm0.008\pm0.002\pm0.019$	&$0.073\pm0.009\pm0.002\pm0.012$	&$-$	\\
$[8,9]$&$0.086\pm0.009\pm0.003\pm0.011$	&$0.067\pm0.006\pm0.002\pm0.014$	&$0.050\pm0.006\pm0.001\pm0.010$	&$0.031\pm0.006\pm0.001\pm0.005$	&$-$	\\
$[9,10]$&$0.052\pm0.007\pm0.002\pm0.007$	&$0.044\pm0.005\pm0.001\pm0.009$	&$0.027\pm0.004\pm0.001\pm0.006$	&$0.026\pm0.006\pm0.002\pm0.004$	&$-$	\\
$[10,12]$&$0.027\pm0.004\pm0.001\pm0.004$	&$0.020\pm0.002\pm0.001\pm0.004$	&$0.020\pm0.002\pm0.001\pm0.004$	&$-$	&$-$	\\
$[12,14]$&$0.012\pm0.002\pm0.001\pm0.002$	&$0.007\pm0.002\pm0.000\pm0.001$	&$0.008\pm0.002\pm0.000\pm0.002$	&$-$	&$-$	\\
\hline
Backward&&&&&\\
$\pt[\gevc]$ &$-3.0<y^*<-2.5$   &$-3.5<y^*<-3.0$    &$-4.0<y^*<-3.5$     &$-4.5<y^*<-4.0$     &$-5.0<y^*<-4.5$\\
\hline
$[0,1]$&$-$	&$3.749\pm0.796\pm0.164\pm0.556$	&$3.461\pm0.780\pm0.127\pm0.351$	&$6.190\pm1.561\pm0.314\pm1.169$	&$-$	\\
$[1,2]$&$6.929\pm0.818\pm0.212\pm1.243$	&$6.020\pm0.400\pm0.086\pm0.777$	&$7.245\pm0.440\pm0.103\pm0.655$	&$5.443\pm0.549\pm0.107\pm0.678$	&$1.654\pm0.877\pm0.129\pm0.202$	\\
$[2,3]$&$4.441\pm0.305\pm0.075\pm0.723$	&$4.488\pm0.181\pm0.044\pm0.469$	&$3.931\pm0.157\pm0.039\pm0.369$	&$2.883\pm0.182\pm0.044\pm0.268$	&$1.519\pm0.265\pm0.050\pm0.205$	\\
$[3,4]$&$2.270\pm0.137\pm0.032\pm0.293$	&$2.062\pm0.082\pm0.019\pm0.235$	&$1.559\pm0.068\pm0.016\pm0.182$	&$0.955\pm0.065\pm0.014\pm0.101$	&$0.358\pm0.093\pm0.014\pm0.043$	\\
$[4,5]$&$1.077\pm0.070\pm0.017\pm0.116$	&$0.934\pm0.045\pm0.011\pm0.127$	&$0.622\pm0.036\pm0.008\pm0.087$	&$0.337\pm0.034\pm0.007\pm0.042$	&$0.232\pm0.053\pm0.011\pm0.027$	\\
$[5,6]$&$0.450\pm0.037\pm0.008\pm0.051$	&$0.377\pm0.025\pm0.005\pm0.059$	&$0.290\pm0.022\pm0.005\pm0.046$	&$0.166\pm0.020\pm0.004\pm0.024$	&$-$	\\
$[6,7]$&$0.265\pm0.026\pm0.006\pm0.032$	&$0.208\pm0.017\pm0.004\pm0.036$	&$0.154\pm0.015\pm0.004\pm0.025$	&$0.053\pm0.011\pm0.002\pm0.008$	&$-$	\\
$[7,8]$&$0.125\pm0.015\pm0.003\pm0.017$	&$0.059\pm0.008\pm0.001\pm0.011$	&$0.052\pm0.009\pm0.002\pm0.009$	&$0.038\pm0.011\pm0.002\pm0.006$	&$-$	\\
$[8,9]$&$0.074\pm0.010\pm0.003\pm0.010$	&$0.042\pm0.008\pm0.001\pm0.008$	&$0.022\pm0.006\pm0.001\pm0.004$	&$-$	&$-$	\\
$[9,10]$&$0.043\pm0.009\pm0.002\pm0.007$	&$0.027\pm0.005\pm0.001\pm0.005$	&$-$	&$-$	&$-$	\\
$[10,14]$&$0.010\pm0.002\pm0.000\pm0.002$	&$0.007\pm0.001\pm0.000\pm0.002$	&$-$	&$-$	&$-$	\\


==> tablesDs/p_CrossSection1DPT.tex <==
Forward [\mbarn/(\gevc)] &&&&&\\
$\pt[\gevc]$&$1.5<y^*<4.0$ &$2.5<y^*<4.0$ &$3.0<y^*<4.0$ &$2.5<y^*<3.5$ &$2.5<y^*<3.0$\\
\hline
$[0,1]$&$6.239\pm0.526\pm0.511$&$4.522\pm0.484\pm0.426$&$0.730\pm0.148\pm0.076$&$-$	&$-$	\\
$[1,2]$&$12.855\pm0.387\pm0.693$&$7.433\pm0.249\pm0.381$&$-$	&$-$	&$-$	\\
$[2,3]$&$8.344\pm0.167\pm0.442$&$4.210\pm0.105\pm0.213$&$-$	&$-$	&$-$	\\
$[3,4]$&$4.041\pm0.073\pm0.195$&$1.970\pm0.048\pm0.100$&$-$	&$-$	&$-$	\\
$[4,5]$&$1.988\pm0.041\pm0.098$&$0.925\pm0.026\pm0.048$&$-$	&$-$	&$-$	\\
$[5,6]$&$0.998\pm0.027\pm0.051$&$0.425\pm0.019\pm0.023$&$-$	&$-$	&$-$	\\
$[6,7]$&$0.488\pm0.018\pm0.026$&$0.226\pm0.014\pm0.013$&$-$	&$-$	&$-$	\\
$[7,8]$&$0.230\pm0.010\pm0.011$&$0.092\pm0.006\pm0.005$&$-$	&$1.000\pm0.135\pm0.067$&$-$	\\
$[8,9]$&$0.125\pm0.007\pm0.007$&$0.047\pm0.004\pm0.003$&$-$	&$0.774\pm0.120\pm0.058$&$-$	\\
$[9,10]$&$0.078\pm0.006\pm0.005$&$0.029\pm0.004\pm0.003$&$-$	&$0.775\pm0.163\pm0.077$&$-$	\\
$[10,12]$&$0.035\pm0.003\pm0.002$&$0.011\pm0.001\pm0.001$&$-$	&$-$	&$1.472\pm0.381\pm0.121$\\
$[12,14]$&$0.015\pm0.002\pm0.001$&$0.004\pm0.001\pm0.000$&$-$	&$-$	&$0.000\pm0.000\pm-1.000$\\
\hline
Backward [\mbarn/(\gevc)]&&&&&\\
$\pt[\gevc]$&$-5.0<y^*<-2.5$ &$-4.0<y^*<-2.5$ &$-4.0<y^*<-3.0$ &$-3.5<y^*<-2.5$ &$-3.0<y^*<-2.5$\\
\hline
$[0,1]$&$6.757\pm0.737\pm0.607$&$4.116\pm0.506\pm0.331$&$0.730\pm0.148\pm0.062$&$-$	&$-$	\\
$[1,2]$&$15.462\pm0.694\pm1.088$&$11.204\pm0.554\pm0.817$&$-$	&$-$	&$-$	\\
$[2,3]$&$9.354\pm0.275\pm0.503$&$6.842\pm0.213\pm0.351$&$-$	&$-$	&$-$	\\
$[3,4]$&$3.754\pm0.114\pm0.195$&$3.055\pm0.100\pm0.157$&$-$	&$-$	&$-$	\\
$[4,5]$&$1.710\pm0.060\pm0.082$&$1.375\pm0.048\pm0.063$&$-$	&$-$	&$-$	\\
$[5,6]$&$0.700\pm0.029\pm0.036$&$0.607\pm0.027\pm0.031$&$-$	&$-$	&$-$	\\
$[6,7]$&$0.371\pm0.019\pm0.018$&$0.342\pm0.019\pm0.017$&$-$	&$-$	&$-$	\\
$[7,8]$&$0.125\pm0.011\pm0.008$&$0.125\pm0.011\pm0.008$&$-$	&$1.000\pm0.135\pm0.077$&$-$	\\
$[8,9]$&$0.073\pm0.008\pm0.004$&$0.073\pm0.008\pm0.004$&$-$	&$0.774\pm0.120\pm0.058$&$-$	\\
$[9,10]$&$0.038\pm0.006\pm0.004$&$0.038\pm0.006\pm0.004$&$-$	&$0.775\pm0.163\pm0.061$&$-$	\\
$[10,14]$&$0.009\pm0.001\pm0.001$&$0.009\pm0.001\pm0.001$&$-$	&$-$	&$1.472\pm0.381\pm0.119$\\

